Recurrent neural networks approximate continuous functions

Classical approximation theorems ask for a new neural network whenever the target accuracy is improved. This paper studies the opposite possibility: can the network be chosen once and for all, and can accuracy be bought only by letting it run longer? We prove that this is possible for every continuous function on [-1,1]. More precisely, each such function is uniformly approximated by the time evolution of a single ReLU recurrent neural network with fixed weights and fixed hidden dimension. The mechanism behind the construction is a new intermediate model, the Turing machine with neural units (TMNU). This model retains the algorithmic freedom needed to implement polynomial approximation schemes, while remaining rigid enough to be simulated by RNNs with explicit bounds on hidden dimension and weight magnitude. The resulting convergence rates reflect the underlying polynomial approximation rates. We complement the construction with minimax lower bounds showing that runtime is not merely a proof artifact, but an unavoidable resource in this fixed-network approximation paradigm.

==> LatexCommands/customPackages/physicalUnits.tex <==
%%%%% Unit Denominators %%%%%%%%%%
\newcommand\dB{\ensuremath{\,\mathrm{dB}}}
\newcommand\dBm{\ensuremath{\,\mathrm{dBm}}}
\newcommand\Hz{\ensuremath{\,\mathrm{Hz}}}
\newcommand\kHz{\ensuremath{\,\mathrm{kHz}}}
\newcommand\MHz{\ensuremath{\,\mathrm{MHz}}}
\newcommand\GHz{\ensuremath{\,\mathrm{GHz}}}
\newcommand\s{\ensuremath{\,\mathrm{s}}}
\newcommand\ms{\ensuremath{\,\mathrm{ms}}}
\newcommand\mus{\ensuremath{\,\mathrm{\text{\textmu}s}}}
\newcommand\ns{\ensuremath{\,\mathrm{ns}}}
\newcommand\ps{\ensuremath{\,\mathrm{ps}}}
\newcommand\meter{\ensuremath{\,\mathrm{m}}}
\newcommand\mm{\ensuremath{\,\mathrm{mm}}}
\newcommand\cm{\ensuremath{\,\mathrm{cm}}}
\newcommand\m{\ensuremath{\,\mathrm{m}}}
\newcommand\W{\ensuremath{\,\mathrm{W}}}
\newcommand\mW{\ensuremath{\, \mathrm{mW}}}
\newcommand\J{\ensuremath{\,\mathrm{J}}}
\newcommand\K{\ensuremath{\,\mathrm{K}}}
\newcommand\bit{\ensuremath{\,\mathrm{bit}}}
\newcommand\nat{\ensuremath{\,\mathrm{nat}}}

==> LatexCommands/packages_beamer.tex <==
%%% This file imports all useful packages

% manage different pdf files
\usepackage{hyperref} % gestion of hypertext links

%packages for encoding languages
\usepackage[english]{babel} %gestion of english characters
\usepackage[utf8]{inputenc}  % The package translates various standard and other input encodings into a ‘LaTeX internal language’.
\usepackage[T1]{fontenc}  % The package allows the user to select font encodings
\usepackage{lmodern} %vectorial characters
\usepackage{relsize} %have better character sizes


%helps having good presentation
\usepackage{fancyhdr} %to have a fancy presentation of the article (headers, titles...)
\usepackage{geometry} %to have a good page layout
\usepackage{xspace} % tool to help not having undesired spaces in the document
\usepackage{enumitem} %to make enumerations, itemize, etc
\usepackage{tcolorbox} %to make boxes that are easy to see

% emphasizing text (bold, underlining, letterspacing)
\usepackage{soul} %basic stuff
\usepackage[normalem]{ulem} %more precise entries


% to make cool figures
\usepackage{float} % most flexible package to make figures out of nothing
\usepackage{graphicx} % used to insert images (the easiest tool to use)
\usepackage{wrapfig} % makes figures in any way wanted (very precise precision etc) 
\usepackage{caption, subcaption} % use to caption figures
\usepackage{multirow} % used to modify tables with high flexibility
\usepackage{media9} %used to have animated 3D objects, sounds, etc
\usepackage{transparent} % used to make elements transparent
\usepackage[dvipsnames, x11names]{xcolor} %use to change color of figures

% to make custom commands
\usepackage{xargs, xparse} % handles multiple optional parameters 

%testing commands
\usepackage{blindtext} %creates random text
\usepackage{comment} %to make commentaries

% usage of functions within the latex code
\usepackage{ifthen} %to be able to use boolean propositions in the latex code
\usepackage{expl3} %to make more complex boolean logic operations
\usepackage{multido} %be able to make code loops

% usage of comments
\usepackage{pdfcomment}

%type math symbols, equations
\usepackage{amsmath,amssymb,mathrsfs,mathtools, amsthm, amsbsy} % packages of mathematical symbols
\usepackage{empheq} %extension of amsmath
\usepackage{esint} %integral symbols
\usepackage{siunitx} %write numbers in scientific writing
\usepackage{cancel} %to bar some expressions
\usepackage{cases} % to make case by case equations
\usepackage{mdframed} % allows to frame equations
\usepackage{bm, bbm} %to type bold math fonts
\usepackage{upgreek} % to type non italic versions of greek letters
\usepackage{mleftright} % makes a better displaying for parentheses

%drawing graphs
\usepackage{tikz}%automatically draw math functions
\usepackage{pgfplots}%automatically draw math functions
\usetikzlibrary{plotmarks} %initiates tikz
\pgfplotsset{compat=1.14} %initiates pgfplot
\usetikzlibrary{math} %to perform math operations in latex
\usetikzlibrary{decorations.pathreplacing,shapes,shapes.misc} %to make shapes and decorations

%algorithmy
\usepackage{algorithm, algpseudocode} %to make algorithms

%make nice references to equations, etc
\usepackage{cleveref} % make nice references


%%%%%%% Custom packages %%%%%%%%%%

\input{customPackages/basicMacros}
% \input{customPackages/theorems}
\input{customPackages/customFonts}
\input{customPackages/basicMathMacros}
\input{customPackages/polynomes}
\input{customPackages/symbolicSequences}
\input{customPackages/computableAnalysis}
\input{customPackages/betaExpansions}


==> subfiles/intro/intro.tex <==
% TEX root = main.tex


\chapter{Introduction}

\section{Story}
In a famous paper, \cite{cybenkoApproximationSuperpositionsSigmoidal} shows that for every continuous function, and every $\varepsilon > 0$, there exists a neural network that approximates this function within precision $\varepsilon$. While providing this general result, the proof is not constructive. Since then, a large body of literature has been dedicated to make constructive proofs of the neural networks that can approximate continuous functions. \cite{elbrachter2021DeepNeuralNetworka} systematically studies the approximation of polynomials with neural networks of minimal size. For instance, the function $\realx \mapsto \realx^2$ can be approximated over $[-1,1]$ with precision $\varepsilon > 0$ by means of a neural network of length $O(\log(1/\varepsilon))$ and of width $4$. Still, this shows that in order to approximate a continuous function, one needs a neural network of a size that grows with the precision $\varepsilon$. 

In this paper, we turn to Recurrent Neural Networks (\RNNs). The principle of an \RNN is to take a neural network and use it as a recursive function, i.e. to use the output of the neural network as an input for the next step. The goal of this paper is to show that \RNNs can approximate continuous functions with a fixed size, independently of the precision $\varepsilon$. The need to increase the size of the neural network for better precision is replaced by the need to increase the number of steps performed by the \RNN. To be clearer, let us state an informal version of this result in mathematical symbols. The formal version of the result appears later in the paper. For an \RNN $\rnn$ to which we feed an input $\realx \in \R$, the output of the \RNN at time step $t \in \No$ is denoted by $\rnn\realx[t] \in \R$. 
\begin{theorem} (Informal)
    Let $f : \Omega \to \R$ be a continuous function defined on a compact subset $\Omega$ of $\R$. Then, there exists an \RNN $\rnn$ such that
    \begin{equation}
       \limi{t} \left|\rnn\realx[t] - f(\realx)\right| = 0.
    \end{equation}
\end{theorem}

The scope of our paper is not limited to this theorem. The novelty of this work resides also in the method deployed to achieve this proof. Namely, we introduce a new model of computation, the Turing Machine with Neural Units (\TMNU). Before explaining what \TMNUs consist of, let us first explain why such a model naturally arises in the context of \RNNs. \RNNs have been famously proven to be Turing complete, by a clever construction to simulate Turing machines with \RNNs \cite{siegelmann1992ComputationalPower}. This construction has been pushed slightly further in \cite{balcazar1997ComputationalPowerNeural}, that establishes that \RNNs can simulate oracle Turing machines \cite[Section V]{balcazar1997ComputationalPowerNeural}. The equivalence of \RNNs and oracle Turing machines already yields an important result when put in perspective with the theory of computable analysis \cite{weihrauch2000ComputableAnalysis}. Given a real function $f: \R \to \R$ and a way of encoding real numbers into infinite binary strings, say through a surjective map $\eta : \{0,1\}^\N \to \R$, we can associate a function acting on infinite binary strings $F : \{0,1\}^\N \to \{0,1\}^\N$ that realizes the function $f$ in the sense that
\begin{equation}
    \eta(F(\sequ)) = f(\eta(\sequ)), \quad \forall \sequ \in \{0,1\}^\N.
\end{equation}
Then, one of the standard results of computable analysis is that when $\eta$ is chosen to be a specific representation called the Cauchy representation, every continuous function can be realized by an oracle Turing machine \cite[Theorems 2.3.13, Definition 3.2.7, Theorem 3.2.11, Definition 4.1.3, Lemma 4.1.6]{weihrauch2000ComputableAnalysis}, i.e., for every continuous function $f : \R \to \R$, there exists a function $F : \{0,1\}^\N \to \{0,1\}^\N$ that realizes $f$, such that $F$ can be computed by an oracle Turing machine, thus by an \RNN, since as discussed above, RNNs can simulate oracle Turing machines. This means that through the Cauchy representation, \RNNs can approximate every continuous function if we use the \RNNs as functions acting on infinite binary strings. However, we want to know if \RNNs can approximate continuous functions when we use them as acting on real numbers directly. The framework of Turing machines turned out not to be directly fitted to this question. 

Continuing in the philosophy of simulating machines with \RNNs, one could turn to the simulation of real Turing machines with \RNNs. Real Turing machines, also known as Blum-Shub-Smale machines (BSS machines) \cite{blum1998ComplexityRealComputation}, are a kind of abstract machines that can manipulate real numbers instead of binary strings. However, at the core of the definition of BSS machines, lays the usage of discontinuous threshold functions, making them too powerful to be simulated by \RNNs. Our quest of finding a suitable model of computation that can be simulated by \RNNs and that can manipulate real numbers led us to introduce the Turing Machine with Neural Units (\TMNU). The \TMNU is a Turing machine that has access to a finite set of neural networks. At the beginning of the computation, the \TMNU receives a real number $\realx \in \R$ as input, and then applies to $\realx$, one by one, the different \NNs it has at hand, in an order that is decided by the finite control of the \TMNU. We will introduce the formal definition of \TMNU later in the paper. 

This paper is organized as follows. In Section \ref{sec:turing machine with neural units}, we introduce the Turing Machine with Neural Units (\TMNU) and related concepts such as complexity classes. In Section \ref{sec:TMNU-approximation-of-continuous-functions}, we show that \TMNUs can approximate continuous function and establish the complexity classes associated with continuous functions. In Section \ref{sec:recurrent-neural-networks}, we prove that \RNNs can simulate \TMNUs, thus yielding that \RNNs can approximate continuous functions. Throughout the paper, we also study the complexity classes that naturally arise in the context of \TMNUs and \RNNs.




==> subfiles/notation/notation.tex <==
% TEX root = main.tex

\section{Notation and definitions} \label{sec:notation and definitions}


\subsection{Basic set theory}
\begin{itemize}
	\item $\N := \{1,2,\ldots\}$ denotes the set of natural numbers, $\No := \{0\} \cup \N$ the set of natural numbers including zero, $\Z$ denotes the set of integers, $\Q$ the set of rational numbers, and $\R$ the set of real numbers. For $\realx \in \R$, we let $\lfloor \realx \rfloor$ denote the greatest integer less than or equal to $\realx$, and $\lceil \realx \rceil$ the smallest integer greater than or equal to $\realx$. For $n \in \N$, we let $[n] := \{1, 2, \ldots, n\}$.
	\item Let $A$ be a set and $\circ$ be an internal operation on $A$, that is not necessarily associative. For $a_1, a_2, \ldots, a_n \in A$, we define the notation
	\[
		\bigcirc_{i=1}^n a_i := \begin{cases}
			a_1 & \text{if } n=1,\\
			a_n \circ \left(\bigcirc_{i=1}^{n-1} a_i\right) & \text{if } n>1.
		\end{cases}
	\]
	For $n \geq 2$, we might as well write $a_n \circ \ldots \circ a_1$ instead of the more cumbersome $\bigcirc_{i=1}^n a_i$.
	% \item Let $n \in \N$, $A_1, \ldots, A_n$ be $n$ sets. An \newname{$n$-tuple} is a map $\tuplu : \{1, \ldots, n\} \to \bigcup_{i=1}^n A_i$ such that $\tuplu(i) \in A_i$, for all $i \in \{1, \ldots, n\}$. We denote by $a = (a_1, a_2, \ldots, a_n)$ the $n$-tuple $\tuplu$ such that $\tuplu(i) = a_i$, for all $i \in \{1, \ldots, n\}$. We let $A_1 \times A_2 \times \ldots A_n$ denote the set of $n$-tuples $\tuplu$ such that $\tuplu(i) \in A_i$, for all $i \in \{1, \ldots, n\}$. We generally write $a_1\ldots a_n$ instead of $(a_1, \ldots,a_n)$ when there is no risk of confusion. Let $a = a_1 \ldots a_n$ be an $n$-tuple, and $b = b_1 \ldots b_m$ be an $m$-tuple. Their \newname{concatenation} is the $(n+m)$-tuple $c := a_1 \ldots a_n b_1 \ldots b_m$. 
	\item Let $A,X$ be two sets, such that $X$ is finite or countable. A sequence over $A$ indexed by $X$ is a map $\sequ : X \to A$. We denote by $A^X$ the set of sequences over $A$. We denote by $\varepsilon$ the unique element of $A^\varnothing$. For $\sequ \in A^X$ and $x \in X$, we let $\sequ_x := \sequ(x)$, and if $X = \No$, we will also use the notation $\sequ[t] := \sequ(t)$, for all $t \in \No$. Let $a = a_1\ldots a_n$ be an $n$-tuple, and $\sequ \in A^\N$ be a sequence over $A$. Their \newname{concatenation} is the sequence $\sequ' \in A^{\{1, \ldots, n\} \cup X}$ defined by
	\[
		\sequ'_i := \begin{cases}
			a_i & \text{if } i \in \{1, \ldots, n\},\\
			\sequ_{i-n} & \text{if } i > n.
		\end{cases}
	\]
    \iffalse
	\item Let $d,d' \in \No$, $d \leq d'$. An index injection is an injective map $\indinj : \{1, \ldots, d\} \to \{1,\ldots,d'\}$. Moreover, for $J \subseteq \{1,\ldots,d'\}$ with $|J| = d$, $\indinj_J : \{1, \ldots, d\} \to \{1,\ldots,d'\}$ denotes the index injection that enumerates the elements of $J$ in increasing order, i.e., for all $i \in \{1, \ldots, d\}$, $\indinj_J(i)$ is the $i$-th smallest element of $J$. 
	\item Let $d \in \N$. A permutation of size $d$ is a bijective map $\perm : \{1, \ldots, d\} \to \{1, \ldots, d\}$. For $I,J \subseteq \{1,\ldots,d\}$ with $|I| = |J|$, we let $\perm_{d,I,J}$ be the permutation of size $d$ defined by
	\[
		\perm_{d,I,J}(i) := \begin{cases}
			\indinj_J(\indinj_I^{-1}(i)) & \text{if } i \in I,\\
			i & \text{otherwise},
		\end{cases} \quad \forall i \in \{1, \ldots, d\}.
	\]
    \fi
\end{itemize}

\iffalse
\subsection{Ordered sets}
\begin{itemize}
	\item An \newname{ordered set} is a pair $(A,<)$ where $A$ is a set and $<$ is a binary relation over $A$ that is antisymmetric and transitive. We say that $<$ is a \newname{total order} if for all $a,b \in A$, either $a < b$, $a = b$ or $b < a$. We say that $(A,<)$ is \newname{well-ordered} if $<$ is total and every non-empty subset of $A$ has a minimal element with respect to $<$. We say that $(A,<)$ has \newname{finite rank} if for every $a \in A$, the set $\{b \in A : b < a\}$ is finite.
	\item Let $(A,<)$ be a well-ordered set. For $a \in A$, we define its \newname{successor} $\successor{a} \in A$ as the smallest element of $A$ that is strictly greater than $a$, i.e.,
	\[
		\successor{a} := \min\{b \in A : b > a\}.
	\]
	\item Assume that $A$ is well-ordered. The \newname{increasing enumeration} of $A$ is a map $\eta : \No \to A$ such that $\eta(0)$ is the smallest element of $A$, and for all $n \in \N$, $\eta(n) = \successor{\eta(n-1)}$. 
	\begin{lemma}\label{lem:increasing-enumeration-bijection-finite-rank}
		Let $(A,<)$ be a well-ordered set of finite rank. Then, its increasing enumeration $\eta : \No \to A$ is a bijection.
	\end{lemma}
	\begin{proof}
		By definition of the increasing enumeration, $\eta$ is injective. To show that it is surjective, let $a \in A$. The set $A_a := \{b \in A : b < a\}$ is finite, so it has cardinality $k \in \No$. We prove by induction that $\eta(k+1) = a$. If $k=0$, then $a$ is the smallest element of $A$, and by definition of $\eta$, we have that $\eta(0) = a$. Otherwise, let $b$ be the largest element of $A_a$. Then, $A_b = \{c \in A : c < b\} = A_a \backslash \{b\}$, i.e., the cardinality of $A_b$ is exactly $k-1$.By induction hypothesis, we have that $\eta(k) = \eta(k - 1 + 1) = b$. By definition of the successor, we have that $\eta(k+1) = \successor{b} = a$. This shows that $\eta$ is surjective.
	\end{proof}
	Note that this implies that every well-ordered set of finite rank is countable.
\end{itemize}
\fi

\subsection{Strings and sequences}
\begin{itemize}
	\item We define the \newname{empty sequence} $\emptystr := \varnothing$.
	\item Let $A$ be a set and $n \in \No$. We let $A^n := A^{\{1,\ldots,n\}}$. We further let 
	\[
		A^{\leq n} := \bigcup_{i=0}^n A^i, \ \forall n \in \No,
	\]
	
	\[
		A^\ast := \bigcup_{n \in \No} A^n, \quad \text{and} \quad A^+ := \bigcup_{n \in \N} A^n.
	\]
	% Note that the $A^n$ are disjoint sets. 
    Elements of $A^\ast$ are called \newname{finite sequences} over $A$.
	\item For $\wordw \in A^\ast$, we let $\wordw^0 := \emptystr$ and $\wordw^n := \wordw^{n-1} \wordw$, for $n \in \N$. For instance $0^5 = 00000$, $(10)^3 = 101010$ and $01^4 = 01111$. 
	\item We let $A^\# := A^\ast \cup A^\N$. For $\sequ \in A^\#$, we define its \newname{length} $\len{\sequ}$ as follows:
	\[
		\len{\sequ} := \begin{cases}
			n & \text{if } \sequ \in A^n,\\
			\infty & \text{if } \sequ \in A^\N.
		\end{cases}
	\]
	Given $\wordu, \wordv \in A^\ast$, we say that $\wordu$ is shorter than $\wordv$ if $\len{\wordu} < \len{\wordv}$.
	\item Let $A$ be a set, and $\wordu, \wordv \in A^\ast$. We say that $\wordu$ is a \newname{prefix} of $\wordv$, and write $\wordu \prefix \wordv$, if there exists $\wordw \in A^\ast$ such that $\wordv = \wordu \wordw$. If moreover $\wordu \neq \wordv$, we say that $\wordu$ is a \newname{strict prefix} of $\wordv$. 
	% \item Let $(A,<)$ be an ordered set. We define the \newname{quasilexicographic order} on $A^\ast$, denoted by $\qlexl$, as follows. For $\wordu, \wordv \in A^\ast$, we let $\wordu \qlexl \wordv$ if either $\len{\wordu} < \len{\wordv}$ or if $\len{\wordu} = \len{\wordv}$ and there exists $i \in \{1, \ldots, \len{\wordu}\}$ such that $\wordu_j = \wordv_j$ for all $j < i$ and $\wordu_i < \wordv_i$.
	% \begin{lemma}\label{lem:quasilexicographic-order-well-ordered-finite-rank}
	% 	Let $(A,<)$ be an ordered finite set, such that $<$ is total. Then, $(A^\ast, \qlexl)$ is a well-ordered set of finite rank.
	% \end{lemma}
	% \begin{proof}
	% 	Antisymmetry and transitivity of $\qlexl$ are straightforward. We first show that $\qlexl$ is a total order on $A^\ast$. Let $\wordu, \wordv \in A^\ast$. If $\len{\wordu} < \len{\wordv}$, then $\wordu \qlexl \wordv$. If $\len{\wordu} > \len{\wordv}$, then $\wordv \qlexl \wordu$. Otherwise, $\len{\wordu} = \len{\wordv}$. If $\wordu = \wordv$, then neither $\wordu \qlexl \wordv$ nor $\wordv \qlexl \wordu$ hold. Otherwise, there exists $i \in \{1, \ldots, \len{\wordu}\}$ such that $\wordu_j = \wordv_j$ for all $j < i$ and $\wordu_i \neq \wordv_i$. Since $<$ is total over $A$, either $\wordu_i < \wordv_i$ or $\wordv_i < \wordu_i$. In the first case, we have that $\wordu \qlexl \wordv$, and in the second case, we have that $\wordv \qlexl \wordu$. This shows that $\qlexl$ is total over $A^\ast$. 
		
	% 	We now show that $(A^\ast, \qlexl)$ is well-ordered. Let $B \subseteq A^\ast$ be a non-empty subset. Then, there exists $m \in \No$ such that $B \cap A^{\leq m} \neq \varnothing$. Since $A$ is finite, so is $A^{\leq m}$, and thus $B \cap A^{\leq m}$ has a minimal element with respect to the restriction of $\qlexl$ to $A^{\leq m}$. Let $\wordu$ be this minimal element. We claim that $\wordu$ is also the minimal element of $B$ with respect to $\qlexl$. Indeed, let $\wordv \in B$. If $\len{\wordv} > m$, then $\wordu \qlexl \wordv$. Otherwise, since by definition of $m$, $\wordv \in B \cap A^{\leq m}$, and since $\wordu$ is the minimal element of $B \cap A^{\leq m}$, we have that $\wordu \qlexl \wordv$. This shows that $\wordu$ is the minimal element of $B$.
		
	% 	Finally, we show that $(A^\ast, \qlexl)$ has finite rank. Let $\wordu \in A^\ast$. The set $\{\wordv \in A^\ast : \wordv \qlexl \wordu\}$ is included in the finite set $A^{\leq \len{\wordu}}$, and is thus finite. This shows that $(A^\ast, \qlexl)$ has finite rank.
	% \end{proof}
\end{itemize}
\subsection{Prefix-free encodings and pairing functions over finite sequences}
% \begin{itemize}
	% \item
     Let $A$ be a set, and assume that $0,1 \in A$. For $\wordw \in A^\ast$, we define its \newname{prefix-free encoding} $\prfx{\wordw} \in \{0,1\}^\ast$ by
	\[	\prfx{\wordw} := 1^{\len{\wordw}} 0 \wordw. \]
    \iffalse
	\begin{lemma}\label{lem:prefix-free-encoding}
		For all $\wordu, \wordv \in A^\ast$, 
			\[
				\prfx{\wordu} \prefix \prfx{\wordv} \iff \wordu = \wordv.
			\]
	\end{lemma}
	\begin{proof}
		Let $\wordu, \wordv \in A^\ast$, and assume that $\prfx{\wordu} \prefix \prfx{\wordv}$. By definition of the prefix-free encoding, this means that
		\[	1^{\len{\wordv}} 0 \wordv \prefix 1^{\len{\wordu}} 0 \wordu. \]
		In particular, this yields $1^{\len{\wordv}}0 \prefix 1^{\len{\wordu}}0$, which is satisfied only if $\len{\wordv} = \len{\wordu}$. Thus,
		\[	\wordv \prefix \wordu, \]
		and since $\len{\wordu} = \len{\wordv}$, we get that $\wordu = \wordv$. The converse implication is straightforward.
	\end{proof}
    \fi
\iffalse
	\item Let $A$ be a set, and assume that $0,1 \in A$. We define the \newname{pairing function} $\pairAlg{\cdot} : \left(A^\ast\right)^2 \to A^\ast$ by 
	\[
		\pairAlg{\wordu, \wordv} := \prfx{\wordu} \wordv, \quad \forall \wordu, \wordv \in A^\ast.
	\]
	\begin{lemma}\label{lem:pairing-function-injective}
		$\pairAlg{\cdot}$ is injective over $\left(A^\ast\right)^2$.
	\end{lemma}
	\begin{proof}
		Let $\wordu_1, \wordu_2, \wordv_1, \wordv_2 \in A^\ast$, and assume that
		\[	\pairAlg{\wordu_1, \wordv_1} = \pairAlg{\wordu_2, \wordv_2}. \]
		By definition of the pairing function, this means that
		\[	\prfx{\wordu_1} \wordv_1 = \prfx{\wordu_2} \wordv_2. \]
		In particular, $\prfx{\wordu_1} \prefix \prfx{\wordu_2}$, and by Lemma \ref{lem:prefix-free-encoding}, we get that $\wordu_1 = \wordu_2$. Thus,
		\[	\prfx{\wordu_1} \wordv_1 = \prfx{\wordu_1} \wordv_2, \]
		and by cancelling $\prfx{\wordu_1}$ on both sides, we get that $\wordv_1 = \wordv_2$. This shows that $\pairAlg{\cdot}$ is injective.
	\end{proof}
	We extend the pairing function to $k$-tuples as follows. For $k \geq 3$, and $\wordw^{(1)}, \wordw^{(2)}, \ldots, \wordw^{(k)} \in A^\ast$, we define recursively
	\[	\pairAlg{\wordw^{(1)}, \wordw^{(2)}, \ldots, \wordw^{(k)}} := \pairAlg{\wordw^{(1)}, \pairAlg{\wordw^{(2)}, \ldots, \wordw^{(k)}}}. \]
	Unfolding the recursion, we get the explicit formula: 
	\[
		\pairAlg{\wordw^{(1)}, \wordw^{(2)}, \ldots, \wordw^{(k)}} = \prfx{\wordw^{(1)}} \prfx{\wordw^{(2)}} \ldots \prfx{\wordw^{(k-1)}} \wordw^{(k)}.
	\]
	We also set define $\pairAlg{\wordu} := \wordu$, for all $\wordu \in A^\ast$. 
	% Upon noting then, $\pairAlg{\varepsilon} = \varepsilon$, this induces a definition of $\pairAlg{\cdot}$ on $\bigcup_{k \in \No} \left(A^\ast\right)^k = \left(A^\ast \right)^\ast$.
	For $d \in \N$, we let 
	\[\prefSet{A}{d} := \left\{ \pairAlg{\wordw^{(1)}, \wordw^{(2)}, \ldots, \wordw^{(k)}} : \wordw^{(1)}, \wordw^{(2)}, \ldots, \wordw^{(d)} \in A^\ast\right\}.\] Note that for all $d \in \N$, $\prefSet{A}{d+1} \subsetneq \prefSet{A}{d}$. 
	\begin{lemma}\label{lem:pairing-function-injective-general}
		$\pairAlg{\cdot}$ is injective over $\left(A^\ast\right)^d$, for all $d \in \N$.
	\end{lemma}
	\begin{proof}
		We prove the result by induction on $d$. The base case $d=1$ is trivial. For the inductive step, let $d \geq 1$, and assume that $\pairAlg{\cdot}$ is injective over $\left(A^\ast\right)^d$. Let $\wordw^{(1)}_1, \wordw^{(2)}_1, \ldots, \wordw^{(d)}_1, \wordw^{(1)}_2, \wordw^{(2)}_2, \ldots, \wordw^{(d)}_2 \in A^\ast$, and assume that
		\[
			\pairAlg{\wordw^{(1)}_1, \wordw^{(2)}_1, \ldots, \wordw^{(d)}_1} = \pairAlg{\wordw^{(1)}_2, \wordw^{(2)}_2, \ldots, \wordw^{(d)}_2}.
		\]
		By definition of the pairing function, this means that
		\[
			\prfx{\wordw^{(1)}_1} \pairAlg{\wordw^{(2)}_1, \ldots, \wordw^{(d)}_1} = \prfx{\wordw^{(1)}_2} \pairAlg{\wordw^{(2)}_2, \ldots, \wordw^{(d)}_2}.
		\]
		In particular, $\prfx{\wordw^{(1)}_1} \prefix \prfx{\wordw^{(1)}_2}$, and by Lemma \ref{lem:prefix-free-encoding}, we get that $\wordw^{(1)}_1 = \wordw^{(1)}_2$. Thus,
		\[
			\prfx{\wordw^{(1)}_1} \pairAlg{\wordw^{(2)}_1, \ldots, \wordw^{(d)}_1} = \prfx{\wordw^{(1)}_1} \pairAlg{\wordw^{(2)}_2, \ldots, \wordw^{(d)}_2},
		\]
		and by cancelling $\prfx{\wordw^{(1)}_1}$ on both sides, we get that
		\[
			\pairAlg{\wordw^{(2)}_1, \ldots, \wordw^{(d)}_1} = \pairAlg{\wordw^{(2)}_2, \ldots, \wordw^{(d)}_2}.
		\]
		By the induction hypothesis, we get that $\wordw^{(i)}_1 = \wordw^{(i)}_2$, for all $i \in \{2, \ldots, d\}$. This shows that $\pairAlg{\cdot}$ is injective over $\left(A^\ast\right)^{d+1}$.
	\end{proof}
	By injectivity of $\pairAlg{\cdot}$ over $\left(A^\ast\right)^d$, for all $d \in \N$, we have that for all $\wordu \in \prefSet{A}{d}$, there exists a unique $(\wordu^{(1)}, \wordu^{(2)}, \ldots, \wordu^{(d)}) \in \left(A^\ast\right)^d$ such that
	\[		\pairAlg{\wordu^{(1)}, \wordu^{(2)}, \ldots, \wordu^{(d)}} = \wordu. \]
	This yields the following definition.
	\begin{definition}
		Let $d \in \N$. For $u \in \prefSet{A}{d}$, we uniquely define the strings $u \ci i \in A^\ast$ for $i \in \{1, \ldots, d\}$ by the relation
		\[	u = \pairAlg{u \ci 1, u \ci 2, \ldots, u \ci d}. \]
		We call $u \ci i$ the $i$-th \newname{component} of $u$. Moreover, for $I \subseteq \{1,\ldots, d\}$, we define
		\[	u \ci I := \pairAlg{u \ci i : i \in I}. \]
	\end{definition}
\end{itemize}
\fi

\iffalse
\subsection{Pairing over infinite sequences}
\begin{itemize}
	\item Given a finite set $\{\sequ^{(1)}, \sequ^{(2)}, \ldots, \sequ^{(k)}\} \subseteq \{0,1\}^\N$ of sequences, with $k \geq 2$, we define 
	\begin{equation}
		% \begin{cases}
		% 	\langle \sequ^{(1)}, \sequ^{(2)}\rangle := \sequ^{(1)}_1\sequ^{(2)}_1\sequ^{(1)}_2\sequ^{(2)}_2\sequ^{(1)}_3\sequ^{(2)}_3\ldots \ & \text{if } k=2,\\
		% 	\langle \sequ^{(1)}, \sequ^{(2)}, \ldots, \sequ^{(k)} \rangle = \langle \langle \sequ^{(1)}, \sequ^{(2)}, \ldots, \sequ^{(k-1)} \rangle, \sequ^{(k)} \rangle & \text{if } k \geq 3.
		% \end{cases}
		\langle \sequ^{(1)}, \sequ^{(2)}, \ldots, \sequ^{(k)} \rangle = \sequ^{(1)}_1 \sequ^{(2)}_1 \ldots \sequ^{(k)}_1 \sequ^{(1)}_2 \sequ^{(2)}_2 \ldots \sequ^{(k)}_2 \sequ^{(1)}_3 \sequ^{(2)}_3 \ldots \sequ^{(k)}_3 \ldots
	\end{equation}
	\item Given a countable set of sequences $\{\sequ^{(i)}\}_{i\in \N}$, with $\sequ^{(i)} \in \{0,1\}^{\N}$ for all $i \in \N$, we define
	\begin{equation}
		\langle \{\sequ^{(i)}\}_{i\in \N} \rangle := \sequ^{(1)}_1\sequ^{(1)}_2\sequ^{(2)}_1\sequ^{(1)}_3\sequ^{(2)}_2\sequ^{(3)}_1\ldots
	\end{equation} 
\end{itemize}
\fi
% \subsection{Numbers, encodings, and sequences}
% \begin{itemize}
    \iffalse
	\item We let $\Z$ denote the set of integers, and $\Q$ the set of rational numbers. We let $\R$ denote the set of real numbers. For $\realx \in \R$, we let $\lfloor \realx \rfloor$ denote the greatest integer less than or equal to $\realx$, and $\lceil \realx \rceil$ the smallest integer greater than or equal to $\realx$. 
	
	\item Upon noting that $\{0,1\}$ is a finite ordered set with total order, Lemma \ref{lem:quasilexicographic-order-well-ordered-finite-rank} shows $(\{0,1\}^\ast, \qlexl)$ that is a well-ordered set of finite rank. Thus, by Lemma \ref{lem:increasing-enumeration-bijection-finite-rank}, its increasing enumeration $\eta_{\{0,1\}^\ast} : \No \to \{0,1\}^\ast$ is a bijection. We define a shorthand for $\eta_{\{0,1\}^\ast}$. Specifically, instead of writing $\eta_{\{0,1\}^\ast}(n)$, we write $\Nbit{n}$, for all $n \in \No$. Note that $\Nbit{0} = \emptystr$, $\Nbit{1} = 0$, $\Nbit{2} = 1$, $\Nbit{3} = 00$, $\Nbit{4} = 01$, $\Nbit{5} = 10$, $\Nbit{6} = 11$, and so on. Moreover, we overload the symbol $\bitN{\cdot}$ to denote \newname{also} the inverse $\eta_{\{0,1\}^\ast}^{-1}$. That is, for $\wordw \in \{0,1\}^\ast$, we let $\bitN{\wordw} := \eta_{\{0,1\}^\ast}^{-1}(\wordw)$. Note that $\bitN{\emptystr} = 0$, $\bitN{0} = 1$, $\bitN{1} = 2$, $\bitN{00} = 3$, $\bitN{01} = 4$, $\bitN{10} = 5$, $\bitN{11} = 6$, and so on. This allows us to give short formulas involving encodings and decodings of binary strings and natural numbers. For instance, for all $n \in \No$, the expression
	\[
		\bitN{\Nbit{n}0}
	\]
	denotes the natural number whose binary representation is obtained by appending a $0$ to the binary representation of $n$ (i.e., it is equal to $2n$). We also overload the notation $\prfx{\cdot}$ to denote the prefix-free encoding of natural numbers, defined by
	\[		\pbin{n} := \prfx{\Nbit{n}}, \ \forall n \in \No. \]
	\item Given $n \in\No$, we define $\binN(n)$ to be the binary decomposition of $n$, i.e., $\binN(n)$ is the shortest sequence $u \in \{0,1\}^\ast$ that satisfies
	\[
		n = \sum_{i=0}^{\len u -1} u_{i+1} 2^i.
	\]
	We extend the binary decomposition to integers by defining $\binZ(n) := 0\binN(n)$ if $n \geq 0$, and $\binZ(n) := 1\binN(-n)$, if $n < 0$, for $n \in \Z$. We further define $n \mapsto \pbin{n}$ to be the prefix-free encoding of the integers, defined by 
	\[
		\pbin{n} := \prfx{\binZ(n)}, \ \forall n \in \N.
	\]
	Note that $\len{\pbin{n}} = 2\lfloor \log_2(n) \rfloor + 3$. Conversely, we define a canonical way to decode a binary string into an integer. For $\wordw \in \{0,1\}^\ast$, $\nat{\wordw}$ is the only natural number $n \in \No$ such that $\binN{n} = \wordw$.
    \fi
% \end{itemize}

%  For a countable set $X$, $A^X$ denotes the set of infinite sequences of elements in $A$ indexed by $X$. If $X = \N$ or $\Z$, for $\sequ \in A^X$, we denote by $\sequ_i$ the $i$-th element of $\sequ$, for $i \in X$. Given $(x[t])_{t \geq 0} \in A^\No$, we denote by $x[t]$ the $t$-th element of $(x[t])_{t \geq 0}$, for $t \in \No$. 
% We encode every number $n \in \No$ with the infinite binary sequence $\enc_{\No}(n) := 1^n 0^\infty \in \{0,1\}^\N$. 
% In the sequel, in order to avoid overcrowded equations, we will make the confusion between the number $n$ and its encoding $\enc_{\No}(n)$, i.e., we will write $n$ instead of $\enc_{\No}(n)$. 
% For $\sequ, \seqv \in A^\N$, we let
% \begin{equation}
% 	\sequ|\seqv := \begin{cases}
% 		\sequ_{i+1} & \text{if } i \geq 0,\\
% 		\seqv_{-i} & \text{if } i < 0.
% 	\end{cases}
% \end{equation}

% \subsection{Topology}
% Let $(X, \Tc)$ be a topological space.
% \begin{itemize}
% 	\item We let $\bar{X}$ be the closure of $X$.
% 	\item We define the \newname{limit preimage} of function $f : X \to Y$ at point $b \in \bar{Y}$ as
% 	\[		f^\ast(b) := \{a \in \bar{X} : \lim_{x \to a} f(x) = b\}. \]
% \end{itemize}

\iffalse
\subsection{Asymptotic notations}
Let $(X, \Tc)$ be a topological space with topology $\Tc$, and $f,g : X \ \to \R$, and $a\in \bar{X}$.
\begin{itemize}
	\item We let 
	\[
		\limsup_{x \to a} f(x) := \inf_{\substack{U \in \Tc\\ U \ni a}} \sup_{x \in U \backslash \{a\}} f(x),
	\]
	\item We write $f(x) = \bigO{x \to a}(g(x))$ if 
\[
	\limsup_{x \to a} \frac{|f(x)|}{|g(x)|} < +\infty.
\]
	\item We write $f(x) \smallo{x \to a}(g(x))$ if
\[
	\limsup_{x \to a} \frac{|f(x)|}{|g(x)|} = 0.
\]
	\item Let $Y$ be another topological space, $b \in \bar{Y}$, and $h : X \to Y$ be a continuous function. We write
	\[		f(x) = \underset{h(x) \to b}{\Xc}(g(x)) \]
	if 
	\[		f(x_n) = \underset{n \to \infty}{\Xc}(g(x_n)), \quad \forall (x_n)_{n \in \N} \subseteq X, \ s.t. \ \lim_{n \to \infty} h(x_n) = b, \]
	where $\Xc$ is one of the asymptotic notations $\bigO{}$ or $\smallo{}$.
	\item If $Y \subseteq \R^d$ with $(\infty, \ldots, \infty) \in \bar Y$, we abbreviate
	\[
		f(x_1,\ldots,x_d) = \underset{(h_1(x_1),\ldots,h_d(x_d)) \to (\infty,\ldots, \infty)}{\Xc}(g(x_1,\ldots,x_d))
	\]
	by
	\[
		f(x_1,\ldots,x_d) = \underset{h_1(x_1),\ldots,h_d(x_d) \to (\infty,\ldots, \infty)}{\Xc}(g(x_1,\ldots,x_d)),
	\]
	where $\Xc$ is one of the asymptotic notations $\bigO{}$ or $\smallo{}$.
	\item Let $g_1,\ldots,g_k : X \to \R$ and $h : X \to Y$. We abbreviate
	\[		f(x) = \underset{h(x) \to b}{\Xc}(\max\{g_1(x), g_2(x), \ldots, g_k(x)\}) \]
	by
	\[		f(x) = \underset{h(x) \to b}{\Xc}(g_1(x), g_2(x), \ldots, g_k(x)), \]
	where $\Xc$ is one of the asymptotic notations $\bigO{}$ or $\smallo{}$.
	\begin{lemma}\label{lem:summing small o}
		Let $f,g,h : \No \to \R$, and assume that $h(n) \geq 0$ for all $n \in \No$, and that 
		\[
			\lim_{n \to \infty} \sum_{j=0}^n h(j) = +\infty.
		\]
		Then, 
		\[
			f(n) = g(n) + \smallo{n \to \infty}(h(n)) \implies \sum_{j=0}^n f(j)  = \sum_{j=0}^n g(j) + \smallo{n \to \infty}\left( \sum_{j=0}^n h(j) \right).
		\]
	\end{lemma}
	\begin{proof}
		Let $\varepsilon > 0$. By assumption, there exists $N \in \No$ such that for all $n \geq N$, we have that
		\[
			|f(n) - g(n)| \leq \varepsilon h(n).
		\]
		Thus, for all $n \geq N$, we have that
		\[
			\left| \sum_{j=0}^n f(j) - \sum_{j=0}^n g(j) \right| \leq \sum_{j=0}^{N-1} |f(j) - g(j)| + \sum_{j=N}^n |f(j) - g(j)| \leq C + \varepsilon \sum_{j=0}^n h(j),
		\]
		where $C := \sum_{j=0}^{N-1} |f(j) - g(j)|$. Since $\lim_{n \to \infty} \sum_{j=0}^n h(j) = +\infty$, this shows that
		\[
			\frac{\left|\sum_{j=0}^n f(j) - \sum_{j=0}^n g(j)\right|}{\sum_{j=0}^n h(j)} \leq \varepsilon.
		\]
		Since this holds for all $\varepsilon > 0$, we get the desired result.
	\end{proof}
\end{itemize}
\fi

\subsection{Set theory, index injections, projections, and embeddings}

Let $X$ be a set. For $n \in \No$, we denote by $X^n$ the set of $n$-tuples of elements of $X$, i.e., $X^n := \{(x_1, \ldots, x_n) \mid x_i \in X \text{ for all } i = 1, \ldots, n\}$. By convention, we let $X^0 := \{\varnothing\}$ be the singleton containing the empty tuple, such that $X^n \times X^0 = X^0 \times X^n = X^n$ for all $n \in \No$. Specifically, for every $(x_1,\ldots,x_n) \in X^n$, we have $(x_1,\ldots,x_n,\varnothing) = (\varnothing, x_1,\ldots,x_n) = (x_1,\ldots,x_n)$.

\begin{definition}(Identity)\label{def:identity}
    Let $X$ be a set. We define the \newname{identity} on $X$ as the map $\id_X : X \to X$ such that $\id_X(x) = x$ for all $x \in X$. When the context is clear, we will simply write $\id$ instead of $\id_X$.
\end{definition}




\begin{definition}(Index injection)\label{def:index-injection}
    Let $n, m \in \No$, with $n \leq m$. An \newname{index injection} is an injective map $\indexFunc : \{1, \ldots, n\} \to \{1, \ldots, m\}$. We write simply $\indexFunc : n \hookrightarrow m$. We say that two index injections $\indexFunc : n \hookrightarrow p$ and $\indexFunc' : m \hookrightarrow p$ are \newname{disjoint} if $\indexFunc(\{1, \ldots, n\}) \cap \indexFunc'(\{1, \ldots, m\}) = \varnothing$. Given two disjoint index injection $\indexFunc : n \hookrightarrow p$ and $\indexFunc' : m \hookrightarrow p$, we define their \newname{union} $\indexFunc \sqcup \indexFunc' : n + m \hookrightarrow p$ as the index injection such that
    \begin{equation}
        (\indexFunc \sqcup \indexFunc')(i) := \begin{cases}
            \indexFunc(i) & \text{if } 1 \leq i \leq n, \\
            \indexFunc'(i - n) & \text{if } n < i \leq n + m.
        \end{cases}
    \end{equation}
\end{definition}

Note that when $n=0$, there is a unique index injection from $\{1, \ldots, 0\} = \varnothing$ to $\{1, \ldots, m\}$, called the \newname{empty index injection}, denoted by $\varnothing : 0 \hookrightarrow m$.


\begin{definition}(Natural index injection)\label{def:natural-index-injection}
    Let $n \in \N$, and $J := \{j_1 < j_2 < \ldots < j_{\card J}\} \subseteq \{1, \ldots, n\}$. We define the \newname{natural index injection into $J$} $\natIndexFunc{n}{J} : \card J \hookrightarrow n$ as the index injection such that
    \begin{equation}
        \natIndexFunc{n}{J}(i) := j_i \text{ for all } i \in \{1, \ldots, \card J\}.
    \end{equation}
    In particular, for $k \leq n$, we abbreviate $\natIndexFunc{n}{\{1, \ldots, k\}}$ as $\natIndexFunc{n}{k}$.
\end{definition}
Note that $\natIndexFunc{n}{n} = \id_{\{1, \ldots, n\}}$, and that $\natIndexFunc{n}{\varnothing}$ is the empty index injection.


\begin{definition}(Natural complement and natural extension)\label{def:natural-complement-extension}
    Let $n, m \in \N$, with $n \leq m$, and let $\indexFunc : \{1, \ldots, n\} \to \{1, \ldots, m\}$ be an index injection. We define the \newname{natural complement} of $\indexFunc$ as the natural index injection into the complement of the image of $\indexFunc$, i.e., 
    \begin{equation}
        \compl\indexFunc := \natIndexFunc{m-n}{\left(\{1, \ldots, m\} \setminus \indexFunc(\{1, \ldots, n\})\right)}.
    \end{equation}
    Moreover, we define the \newname{natural extension} of $\indexFunc$ as the map 
    \begin{equation}\label{eq:natural-extension:def:natural-complement-extension}
        \exte\indexFunc := \indexFunc \sqcup \compl\indexFunc.
    \end{equation}
\end{definition}

Note that by construction, $\compl\indexFunc$ is an index injection and $\exte\indexFunc$ is a bijection from $\{1, \ldots, m\}$ to itself. Note also that $\compl\varnothing = \id_{\{1, \ldots, m\}}$ and $\exte\varnothing = \id_{\{1, \ldots, m\}}$.
\begin{lemma}
    Let $n, m \in \N$, with $n \leq m$, and let $\indexFunc : \{1, \ldots, n\} \to \{1, \ldots, m\}$ be an index injection. Then, 
    \begin{equation}
         \exte\indexFunc^{-1} \circ \indexFunc = \natIndexFunc{m}{n}.
    \end{equation}
\end{lemma}
\begin{proof}
    Let $i \in \{1, \ldots, n\}$. We have
    \begin{equation*}
        (\exte\indexFunc^{-1} \circ \indexFunc)(i) = \exte\indexFunc^{-1}(\indexFunc(i)) = \exte\indexFunc^{-1}(\exte\indexFunc(i)) = i = \natIndexFunc{m}{n}(i).
    \end{equation*}
    This concludes the proof.
\end{proof}


\begin{definition}(Projection)\label{def:projection}
    Let $X$ be a set, $n, m \in \No$, with $n \leq m$, and $\indexFunc : \{1, \ldots, n\} \to \{1, \ldots, m\}$ be an index injection. We define the \newname{projection} $\proj_{X,\indexFunc} : X^m \to X^n$ as
    \begin{equation}
        \proj_{X,\indexFunc}(x_1, \ldots, x_m) := \left( x_{\indexFunc(1)}, x_{\indexFunc(2)}, \ldots, x_{\indexFunc(n)} \right) \text{ for all } (x_1, \ldots, x_m) \in X^m.
    \end{equation}
    When the context is clear, we will simply write $\proj_{\indexFunc}$ instead of $\proj_{X,\indexFunc}$.
\end{definition}
Note that when $\indexFunc$ is in particular a bijection, then $\proj_{\indexFunc}$ is also a bijection, and in this case, we have $\proj_{\indexFunc}^{-1} = \proj_{\indexFunc^{-1}}$.
Note also that since $X^0 = \{\varnothing\}$ is a singleton (for any set $X$), the projection $\proj_{\varnothing} : X^m \to X^0$ is the unique map from $X^m$ to a singleton. With this formalism, $X^m \times X^0 = X^0 \times X^m = X^m$, and for every $(x_1,\ldots,x_m) \in X^m$, $(x_1,\ldots,x_m,\varnothing) = (\varnothing, x_1,\ldots,x_m) = (x_1,\ldots,x_m)$. Note that if $X =\R$, then $\proj_{X,\indexFunc}$ is a linear map represented by a matrix in $\{0,1\}^{n \times m}$ with exactly one $1$ in each row, and at most one $1$ in each column. We make the confusion of notation between $\proj_{X,\indexFunc}$ and its matrix representation when $X = \R$. This allows to apply usual linear algebra operations to projections, such as the transpose $\proj_{\indexFunc}^T$. Note that $\proj_{\indexFunc}^T : \R^n \to \R^m$ is the linear map defined by
\begin{equation}
    \proj_{\indexFunc}^T(y_1, \ldots, y_n) := (z_1, \ldots, z_m) \text{ for all } (y_1, \ldots, y_n) \in \R^n,
\end{equation}
where for all $j \in \{1, \ldots, m\}$,
\begin{equation}
    z_j := \begin{cases}
        y_i & \text{if } j = \indexFunc(i) \text{ for some } i \in \{1, \ldots, n\}, \\
        0 & \text{otherwise}.
    \end{cases}
\end{equation}
Such a map is usually referred to as an embedding. We next state two useful lemmas about projections.




\begin{lemma}(Decomposition of disjoint projections)\label{lem:decomposition-projections}
    Let $X$ be a set, $n, m, p \in \No$, with $n \leq m \leq p$, and let $\indexFunc : \{1, \ldots, n\} \to \{1, \ldots, p\}$ and $\indexFunc' : \{1, \ldots, m\} \to \{1, \ldots, p\}$ be two disjoint index injections. Then,
    \begin{equation}\label{eq:main:lem:decomposition-projections}
        \proj_{\indexFunc' \sqcup \indexFunc} = (\proj_{\indexFunc}, \proj_{\indexFunc'}).
    \end{equation}
\end{lemma}
\begin{proof}
    Let $(x_1, \ldots, x_p) \in X^p$. We have
    \begin{align*}
        \proj_{\indexFunc' \sqcup \indexFunc}(x_1, \ldots, x_p) &= \left( x_{(\indexFunc' \sqcup \indexFunc)(1)}, x_{(\indexFunc' \sqcup \indexFunc)(2)}, \ldots, x_{(\indexFunc' \sqcup \indexFunc)(n+m)} \right) \\
        &= \left( x_{\indexFunc(1)}, x_{\indexFunc(2)}, \ldots, x_{\indexFunc(n)}, x_{\indexFunc'(1)}, x_{\indexFunc'(2)}, \ldots, x_{\indexFunc'(m)} \right) \\
        &= \left( \proj_{\indexFunc}(x_1, \ldots, x_p), \proj_{\indexFunc'}(x_1, \ldots, x_p) \right) \\
        &= (\proj_{\indexFunc}, \proj_{\indexFunc'})(x_1, \ldots, x_p).
    \end{align*}
    This concludes the proof.
\end{proof}

\begin{lemma}(Composition of projections)\label{lem:composition-projections}
    Let $X$ be a set, $n, m, p \in \No$, with $n \leq m \leq p$, and let $\indexFunc : \{1, \ldots, n\} \to \{1, \ldots, m\}$ and $\indexFunc' : \{1, \ldots, m\} \to \{1, \ldots, p\}$ be two index injections. Then,
    \begin{equation}\label{eq:main:lem:composition-projections}
        \proj_{\indexFunc' \circ \indexFunc} = \proj_{\indexFunc} \circ \proj_{\indexFunc'}.
    \end{equation}
\end{lemma}
\begin{proof}
    Let $(x_1, \ldots, x_p) \in X^p$. We have
    \begin{align*}
        \proj_{\indexFunc' \circ \indexFunc}(x_1, \ldots, x_p) &= \left( x_{(\indexFunc' \circ \indexFunc)(1)}, x_{(\indexFunc' \circ \indexFunc)(2)}, \ldots, x_{(\indexFunc' \circ \indexFunc)(n)} \right) \\
        &= \left( x_{\indexFunc'(\indexFunc(1))}, x_{\indexFunc'(\indexFunc(2))}, \ldots, x_{\indexFunc'(\indexFunc(n))} \right) \\
        &= \proj_{\indexFunc}\left( x_{\indexFunc'(1)}, x_{\indexFunc'(2)}, \ldots, x_{\indexFunc'(m)} \right) \\
        &= \proj_{\indexFunc} \circ \proj_{\indexFunc'}(x_1, \ldots, x_p).
    \end{align*}
    This concludes the proof.
\end{proof}


\begin{definition}\label{def:filter_matrix}
	Let $d \in \N$ and $\iota: \subseteq \{1, \ldots, d\} \to \{1,\ldots,d\}$ be an index injection. The \newname{filter matrix} associated to $\iota$ is the matrix $\filterMat{\iota} \in \R^{d \times d}$ defined by
	\[		(\filterMat{\iota})_{i,j} := \begin{cases}
		1 & \text{if } i \in \dom \iota \text{ and } j = \iota(i),\\
		0 & \text{otherwise},
	\end{cases} \quad \forall i,j \in \{1,\ldots,d\}. \]
\end{definition}

\begin{lemma}\label{lem:filter_matrix}
	Let $d \in \N$ and $\iota: \subseteq \{1, \ldots, d\} \to \{1,\ldots,d\}$ be an index injection. Then, for all $\realx \in \R^d$, we have that
	\[		(\filterMat{\iota}\realx)_i = \begin{cases}
		\realx_{\iota(i)} & \text{if } i \in \dom \iota,\\
		0 & \text{otherwise}.
	\end{cases}
	\]
\end{lemma}
\begin{proof}
	Let $d \in \N$ and $\iota: \subseteq \{1, \ldots, d\} \to \{1,\ldots,d\}$ be an index injection. Then, for all $\realx \in \R^d$ and all $i \in \{1,\ldots,d\}$, we have that
	\[		(\filterMat{\iota}\realx)_i = \sum_{j=1}^d (\filterMat{\iota})_{i,j} \realx_j = \begin{cases}
		\realx_{\iota(i)} & \text{if } i \in \dom \iota,\\
		0 & \text{otherwise}.
	\end{cases}
	\]
\end{proof}

\subsection{Miscellaneous notations}

\begin{itemize}
	% \item For $x \in \R$, $\ReLU(x) := \max\{x,0\}$. If $x \in \R^d$, then $\ReLU(x)$ is applied component-wise.
	% \item Let $j, k,\ell \in \N$, such that $j \leq k \leq \ell$. For $\realx \in \R^k$, we define $\proj j \realx = (\realx_1, \ldots, \realx_j) \in \R^j$ and $\proji \ell \realx = (\realx_1, \ldots, \realx_k, 0, \ldots, 0) \in \R^\ell$. Furthermore, $\|\realx\|_\infty = \max_{i=1, \dots, d} |\realx_i|$.
	\item Let $n,m \in \N$. $\R^n$ denotes the set of $n$-dimensional real vectors, and $\R^{n \times m}$ denotes the set of $n$-by-$m$ real matrices. For $A \in \R^{n \times m}$, we denote by $A^T$ the transpose of $A$. For $A \in \R^{n \times m}$ and $i \in \{1,\ldots,n\}$, $A_i \in \R^m$ denotes the $i$-th row of $A$, and for $j \in \{1,\ldots,m\}$, $A_{ij} \in \R$ denotes the entry of $A$ in the $i$-th row and $j$-th column. We assimilate a vector $x \in \R^n$ to a matrix in $\R^{n \times 1}$, and we write $x^T$ for the transpose of $x$ seen as a matrix. We define a notion of total ordering on $\R^n$, usually referred to as the lexicographic order, by letting $x < y$ if and only if there exists $i \in \{1,\ldots,n\}$ such that $x_i < y_i$ and $x_j = y_j$ for all $j < i$. We extend this lexicographic order to matrices in $\R^{n \times m}$ by letting $A < B$ if and only if there exists $i \in \{1,\ldots,n\}$ such that $A_i < B_i$ and $A_j = B_j$ for all $j < i$. Given a matrix $A \in \R^{n \times m}$ and a vector $b \in \R^m$, we define the affine map $\affine{A}{b} : \R^n \to \R^m$ as $\affine{A}{b}(x) := Ax + b$ for all $x \in \R^n$. We let $\setAffine{n}{m} := \{\affine{A}{b} : A \in \R^{m \times n}, b \in \R^m\}$ be the set of affine maps from $\R^n$ to $\R^m$. We define an ordering on $\setAffine{n}{m}$ by letting $\affine{A}{b} < \affine{A'}{b'}$ if and only if $A < A'$ or $A = A'$ and $b < b'$.
	\item $\idMat_d\in \R^{d\times d}$ is the $d$-dimensional identity matrix, $1_d \in\R^d$ is the $d$-dimensional vector of ones, $\zeroMat_{d,d'} \in \R^{d \times d'}$ denotes the matrix of zeroes with $d$ rows and $d'$ columns, and $0_d \in \R^d$ denotes the vector of zeroes of size $d$.
	\item Given $A$ a set, $A[X]$ denotes the set of polynomials with coefficients in $A$. 
	% \item Let $d,d' \in \No$, $d \leq d'$, and $\indinj : \{1,\ldots,d\} \to \{1,\ldots,d'\}$ be an index injection. We define the canonical coordinate embedding $\cooEmb{\indinj} \in \R^{d \times d'}$ to be the matrix defined by
	% \[		(\cooEmb{\indinj})_{i,j} := \begin{cases}
	% 		1 & \text{if } j = \indinj(i),\\
	% 		0 & \text{otherwise},
	% 	\end{cases} \quad \forall i \in \{1,\ldots,d\}, \forall j \in \{1,\ldots,d'\}. \]
	% We also define the coordinate projection $\cooPro{\indinj} \in \R^{d' \times d}$ as $\cooPro{\indinj} := \cooEmb{\indinj}^T$.
\end{itemize}


%LIMITE PAR RAPPORT A UNE FONCTION?

\iffalse
\subsection{Neural networks and recurrent neural networks}

We proceed to introduce the definitions related to neural networks and recurrent neural networks.
% Given two sets $X$ and $Y$, $f : X \to Y$ defines a function $f$ that maps the points of $X$ to points of $Y$. We write $f : \subseteq X \to Y$ to denote the fact that $f$ is defined only on a subset of $X$. If $f$ is defined only on a subset $\Omega \subseteq X$, we say that $f(x)$ is not defined for all $x \notin \Omega$.

\begin{definition}\label{def:neural network} (Neural network)
Let $L\in \N$ and $N_0, N_1, \ldots, N_{L}\in \N$. A \newname{neural network (\NN)} $\nn$ is a map $\nn: \R^{N_0} \to \R^{N_L}$ given by
\begin{equation}\label{eq:main:def:neural network}
\nn = \begin{cases}
\begin{array}{lc} W_1, & L=1\\
W_2\circ\ReLU\circ W_1, & L=2\\
W_L\circ\ReLU \circ W_{L-1} \circ \ReLU \circ \dots \circ \ReLU \circ W_{1}, & L\ge3 
\end{array} \end{cases}
\end{equation}
where, for $\ell\in\{1,2,\dots,L\}$, $W_{\ell}\colon \R^{N_{\ell-1}} \to \R^{N_\ell},W_\ell(\realx):=A_\ell \realx + b_\ell$
are the associated affine transformations with matrices $A_{\ell}\in \mathbb{R}^{N_{\ell}\times N_{\ell-1}}$ and (bias) vectors $b_\ell\in \mathbb{R}^{N_\ell}$, and the ReLU activation function $\ReLU$ acts component-wise, i.e., $\ReLU(\realx_1,\dots,\realx_N):=(\ReLU(\realx_1),\dots,\ReLU(\realx_N))$.
We denote by $\nns{d}{d'}$ the set of all neural networks with input dimension $N_0=d$ and output dimension $N_L=d'$. 
\end{definition}


% \begin{definition}[Recurrent neural network]\label{def:rnn}
% 	A \newname{recurrent neural network \RNN} for input dimension $\rnnInDim\in\N$, output dimension $\rnnOutDim \in\N$ and hidden state size $\rnnHidDim\in\N$ is parametrized by two \NNs $\nn_h: \R^{\rnnInDim+\rnnHidDim} \rightarrow \R^\rnnHidDim$ and $\nn_o: \R^\rnnHidDim \rightarrow \R^\rnnOutDim$, and a vector $h_0 \in \R^\rnnHidDim$.
% 	% 
% 	These define the \emph{hidden operator} $\Kc: (\R^\rnnInDim)^{\No} \rightarrow (\R^\rnnHidDim)^{\No}$ mapping an input sequence $(\rnnInSeq[t])_{t\geq 0}$ recursively to the sequence of hidden states $(\rnnHidSeq[t])_{t \geq 0}$ according to
% 	\begin{align}
% 		\rnnHidSeq[-1] & := h_0 \in \R^{\rnnHidDim},               \\
% 		\rnnHidSeq[t]  & = \nn_h \begin{pmatrix}
%             \rnnHidSeq[t-1]\\
%             \rnnInSeq[t]
%         \end{pmatrix},
% 	\end{align}
% 	and the \emph{output mapping} $\Qc: \R^{\rnnHidDim} \rightarrow \R^{\rnnOutDim}$
% 	\[
% 		\Qc(\head) :=  \nn_o(\head)
% 	\]
% 	% 
% 	We define the operator $\diracOp : \rnnInSpace \to \left(\rnnInSpace\right)^{\No}$ by $\diracOp\rnnIn[0] = \rnnIn$, and $\diracOp\rnnIn[t] = 0$ for $t \geq 1$, for every $\rnnIn \in \R^{\rnnInDim}$.
% 	The associated \RNN is the operator $\rnn{}: \R^\rnnInDim \rightarrow (\R^{\rnnOutDim})^{\No}$ given by
% 	\[
% 		\rnn := \Qc \Kc \diracOp,
% 	\]
% 	where $\Qc$ is applied independently at each time-step, i.e. for $\rnnInSeq\in \R^\rnnInDim$
% 	\[
% 		(\rnn \rnnInSeq)[t] =   (\Qc \Kc \diracOp\rnnInSeq)[t] = \Qc\left((\Kc \diracOp \rnnInSeq)[t]\right), \quad \textrm{for } t\in\No.
% 	\]
%     % We can also see the \RNN as a map from $\R^\rnnInDim$ to $\left(\R^\rnnOutDim\right)^{\No}$. For $\rnnIn \in \R^\rnnInDim$,  Then, for $\rnnIn \in \R^\rnnInDim$, we set 
%     % \[
%     %     (\rnn \rnnIn)[t] := (\rnn D \rnnIn)[t], \quad \forall t \in \No.
%     % \]  
% \end{definition}


\begin{definition}[Recurrent neural network]\label{def:rnn}
	A \newname{recurrent neural network \RNN} for input dimension $\rnnInDim\in\N$, output dimension $\rnnOutDim \in\N$ and hidden state size $\rnnHidDim\in\N$ is parametrized by two \NNs $\nn: \R^{\rnnInDim+\rnnHidDim} \rightarrow {\rnnOutDim+\rnnHidDim}$ and a vector $h_0 \in \R^\rnnHidDim$.
	% 
	These define the operators $\Kc: (\R^\rnnInDim)^{\No} \rightarrow (\R^\rnnHidDim)^{\No}$ and $\Rc: (\R^\rnnInDim)^{\No} \rightarrow (\R^\rnnOutDim)^{\No}$ mapping an input sequence $(\rnnInSeq[t])_{t\geq 0}$ recursively to the sequence of hidden states $(\rnnHidSeq[t])_{t \geq 0}$ and $(\rnnOutSeq[t])_{t \geq 0}$, respectively, according to
	\begin{align}
		\rnnHidSeq[-1] & := h_0 \in \R^{\rnnHidDim},               \\
		\begin{pmatrix}
            \rnnHidSeq[t]\\
            \rnnOutSeq[t]
        \end{pmatrix}   & = \nn \begin{pmatrix}
            \rnnHidSeq[t-1]\\
            \rnnInSeq[t]
        \end{pmatrix}.
	\end{align}
	$\Kc$ is called the \emph{hidden operator} and $\Rc$ the \emph{RNN operator}.
	% 
	
    % We can also see the \RNN as a map from $\R^\rnnInDim$ to $\left(\R^\rnnOutDim\right)^{\No}$. For $\rnnIn \in \R^\rnnInDim$,  Then, for $\rnnIn \in \R^\rnnInDim$, we set 
    % \[
    %     (\rnn \rnnIn)[t] := (\rnn D \rnnIn)[t], \quad \forall t \in \No.
    % \]  
\end{definition}

In this paper, we will study a specific case of computations with RNNs, namely, the case where the input to the RNN is a sequence which is non-zero only at time $t=0$. This is formalized by the operator $\diracOp$ defined below.
\begin{definition}\label{def:diracOp}
	We define the operator $\diracOp : \cup_{d \in \N} \R^d \to \cup_{d \in \N} 
	\left(\R^d\right)^{\No}$ such that for every $d \in \N$ and $\rnnIn \in \R^d$, $\diracOp\rnnIn[0] = \rnnIn$, and $\diracOp\rnnIn[t] = 0 \in \R^d$ for $t \geq 1$, for every $\rnnIn \in \R^{\rnnInDim}$.
\end{definition}
Specifically, given an RNN as in Definition \ref{def:rnn}, we will study the operator $\Rc \diracOp : \R^{\rnnInDim} \to (\R^{\rnnOutDim})^{\No}$.

We will need the following lemma.

\begin{lemma}\label{lem:extending-nn-with-zeros}
	Let $d,d_i,d_o \in \N$, and let $\nn : \R^{d+d_i} \to \R^{d+d_o}$ be a \NN. Then, there exist an \NN $\tilde \nn : \R^{d+d_o+d_i} \to \R^{d+d_o+d_i}$ such that for all $h \in \R^d$ and all $x \in \R^{d_i}$, 
	\[
		\tilde \nn \begin{pmatrix}
			h\\
			0_{d_o}\\
			x
		\end{pmatrix} = \begin{pmatrix}
			\nn \begin{pmatrix}
				h\\
				x
			\end{pmatrix}\\
			0_{d_i}
		\end{pmatrix},
	\]
\end{lemma}
\begin{proof}
	Let $L \in \N$, $N_0, N_1, \ldots, N_L \in \N$ and $W_i : x \mapsto A_i x + b_i$ with $A_i \in \R^{N_{i-1} \times N_i}$ and $b_i \in \R^{N_i}$ for $i \in \{1, \ldots, L\}$ be such that
	\[		\nn = W_L \circ \ReLU \circ W_{L-1} \circ \ReLU \circ \ldots \circ \ReLU \circ W_1. \]

	We let $\tilde A_1 := \begin{pmatrix}
		A^{(1)}_1 & 0_{N_1, d_o} & A^{(2)}_1
	\end{pmatrix}$ and $\tilde b_1 := b_1$, where $A^{(1)}_1 \in \R^{N_1 \times d}$ and $A^{(2)}_1 \in \R^{N_1 \times d_i}$ are such that $A_1 = \begin{pmatrix}
		A^{(1)}_1 & A^{(2)}_1
	\end{pmatrix}$. We further let $\tilde A_L := \begin{pmatrix}
		A_L\\
		0_{d_i, N_{L-1}}
	\end{pmatrix}$ and $\tilde b_L := \begin{pmatrix}
		b_L\\
		0_{d_i}
	\end{pmatrix}$. Finally, for $i \in \{2, \ldots, L-1\}$, we let $\tilde A_i := A_i$ and $\tilde b_i := b_i$.
	
	Now, for $i \in \{1, \ldots, L\}$, let $\tilde W_i: x \mapsto \tilde A_i x + \tilde b_i$. We define the \NN $\tilde \nn : \R^{d + d_o + d_i} \to \R^{d + d_o + d_i}$ as
	\[		\tilde \nn := \tilde W_L \circ \ReLU \circ \tilde W_{L-1} \circ \ReLU \circ \ldots \circ \ReLU \circ \tilde W_1. \]
	
	Note that for all $h \in \R^d$, $x \in \R^{d_i}$ and $y \in \R^{d_o}$, we have that
	\[
		\tilde W_1 \begin{pmatrix}
			h\\
			y\\
			x
		\end{pmatrix} = \tilde A_1 \begin{pmatrix}
			h\\
			y\\
			x
		\end{pmatrix} + \tilde b_1 = A_1 \begin{pmatrix}
			h\\
			x
		\end{pmatrix} + b_1 = W_1 \begin{pmatrix}
			h\\
			x
		\end{pmatrix}.
	\]
	Similarly, for all $z \in \R^{N_{L-1}}$,
	\[
		\tilde W_L(z) = \tilde A_L z + \tilde b_L = \begin{pmatrix}
			A_L z + b_L\\
			0_{d_i}
		\end{pmatrix} = \begin{pmatrix}
			W_L(z)\\
			0_{d_i}
		\end{pmatrix}.
	\]
	Thus, for all $h \in \R^d$ and all $x \in \R^{d_i}$,
	\[		\tilde \nn \begin{pmatrix}
			h\\
			y\\
			x
		\end{pmatrix} = \tilde W_L \circ \ReLU \circ \tilde W_{L-1} \circ \ReLU \circ \ldots \circ \ReLU \circ \tilde W_1 \begin{pmatrix}
			h\\
			y\\
			x
		\end{pmatrix} = \begin{pmatrix}
			W_L(\ReLU \circ \tilde W_{L-1} \circ \ReLU \circ \ldots \circ \ReLU \circ W_1 \begin{pmatrix}
			h\\
			x
		\end{pmatrix})\\
			0_{d_i}
		\end{pmatrix}
		=
		\begin{pmatrix}
			\nn \begin{pmatrix}
				h\\
				x
			\end{pmatrix}\\
			0_{d_i}
		\end{pmatrix}.
	\]	
\end{proof}


\begin{definition}\label{def:filter_matrix}
	Let $d \in \N$ and $\iota: \subseteq \{1, \ldots, d\} \to \{1,\ldots,d\}$ be an index injection. The \newname{filter matrix} associated to $\iota$ is the matrix $\cooPro{\iota} \in \R^{d \times d}$ defined by
	\[		(\cooPro{\iota})_{i,j} := \begin{cases}
		1 & \text{if } i \in \mathrm{Dom}(\iota) \text{ and } j = \iota(i),\\
		0 & \text{otherwise},
	\end{cases} \quad \forall i,j \in \{1,\ldots,d\}. \]
\end{definition}

\begin{lemma}\label{lem:filter_matrix}
	Let $d \in \N$ and $\iota: \subseteq \{1, \ldots, d\} \to \{1,\ldots,d\}$ be an index injection. Then, for all $\realx \in \R^d$, we have that
	\[		(\cooPro{\iota}\realx)_i = \begin{cases}
		\realx_{\iota(i)} & \text{if } i \in \mathrm{Dom}(\iota),\\
		0 & \text{otherwise}.
	\end{cases}
	\]
\end{lemma}
\begin{proof}
	Let $d \in \N$ and $\iota: \subseteq \{1, \ldots, d\} \to \{1,\ldots,d\}$ be an index injection. Then, for all $\realx \in \R^d$ and all $i \in \{1,\ldots,d\}$, we have that
	\[		(\cooPro{\iota}\realx)_i = \sum_{j=1}^d (\cooPro{\iota})_{i,j} \realx_j = \begin{cases}
		\realx_{\iota(i)} & \text{if } i \in \mathrm{Dom}(\iota),\\
		0 & \text{otherwise}.
	\end{cases}
	\]
\end{proof}

\begin{definition}\label{def:set-injection}
	Let $d \in \N$ and $I \subseteq \{1,\ldots,d\}$. We define the index injection $d|I : I \to \{1,\ldots,d\}$ as $d|I(i) := i$ for all $i \in I$.
\end{definition}
Note that by Lemma \ref{lem:filter_matrix}, for all $d \in \N$, $I \subseteq \{1,\ldots,d\}$, and $\realx \in \R^d$, we have that
\[	(\cooPro{d|I}\realx)_i  = \begin{cases}
		\realx_{i} & \text{if } i \in I,\\
		0 & \text{otherwise}.
	\end{cases}
\]

\fi

==> subfiles/rnn-and-simulation-of-tmnu.tex <==
% TEX root = main.tex

\chapter{\RNNs simulate \TMNUs}

\label{sec:recurrent-neural-networks}

In this section, we show that we can simulate \TMNUs with \RNNs. This results on the establishment of the main result of the paper, i.e., that \RNNs can approximate continuous functions. To this end, we will use the fact that \RNNs can simulate Turing machines, as established in \cite{siegelmann1992ComputationalPower}. We will first recall the construction of the \RNN that simulates a Turing machine, and then we will show how to adapt it to simulate \TMNUs.

\subsection{Simulation of Turing machines by \RNNs}
\label{sec:simulation-turing-machines-rnns}

In this section, we recall the well-known fact that \RNNs can simulate Turing machines, established in \cite{siegelmann1992ComputationalPower}. We give only an overview of the construction. To avoid unnecessary technicalities, we will consider Turing machines that can only contain $0$ or $1$ in their cells (no blank cells). For more details on how to simulate Turing machines with multiple symbols, we refer to \cite{siegelmann1992ComputationalPower}. As a further simplification, we will not really construct the \RNN, but rather we will show that a \TM can be simulated by iteration of a neural network $\nn$. The fact of turning this neural network into an \RNN is also detailed in \cite{siegelmann1992ComputationalPower}. We now proceed to explaining this construction.

Consider a Turing machine $\tm = (n_Q,\transFunc)$. The evolution of the Turing machine is completely described by the sequences $(\trajState{}{t}{},\trajTape{}{t}{},\trajHead{}{t}{})_{t \in \N_0}$ of states, tapes and head positions. We first note that the sequence $(\trajTape{}{t}{}, \trajHead{}{t}{})_{t \in \N_0}$ has an equivalent description: consider the sequences $(\trajTape{L}{t}{}, \trajTape{R}{t}{})_{t \in \N_0}$, satisfying $\trajTape{L}{t}{}, \trajTape{R}{t}{}\in \symbols^\N$ for $t \in \N_0$, such that $\trajTape{L}{t}{}$ contains the symbols of $\trajTape{}{t}{}$ that are located strictly to the left of the head position, and $\trajTape{R}{t}{}$ contains the symbols of $\trajTape{}{t}{}$ that are located to the right of the head position, including the symbol at the head position. In mathematical symbols, this expressed as
\begin{equation}
    \trajCell{L}{t}{}{i} = \trajCell{}{t}{}{{\trajHead{}{t}{}-i}}, \quad \trajCell{R}{t}{}{i} = \trajCell{}{t}{}{{\trajHead{}{t}{}+i-1}}, \quad \forall i \in \N, \quad t \in \N_0.
\end{equation}
The sequence $(\trajState{}{t}{}, \trajTape{L}{t}{}, \trajTape{R}{t}{})_{t \in \N_0}$ is a perfectly valid nonambiguous description of the evolution Turing machine. Based on this alternative description, we will construct a \NN $\nn : \R^{\nStates + 2} \to \R^{\nStates + 2}$ that simulates the Turing machine $\tm$. Specifically, we create a sequence $(\rnnHidSeq[t])_{t \in \No} \in \R^{\nStates + 2}$ that encodes the description $(\trajState{}{t}{}, \trajTape{L}{t}{}, \trajTape{R}{t}{})_{t \in \N_0}$ of the evolution of the \TM. For $t \in \No$, the first $n_Q$ coordinates of $\rnnHidSeq[t]$ store the current state $\trajState{}{t}{}$, while the last two coordinates are used in coordination to simulate the tape of the Turing machine. Concretely, we have
\begin{equation}
    \rnnHidSeq[t] = \begin{pmatrix}
        1_{n_Q, \trajState{}{t}{}} \\
        \cantor(\trajTape{L}{t}{}) \\
        \cantor(\trajTape{R}{t}{})
    \end{pmatrix}, \quad \forall t \in \N_0,
\end{equation}
where $1_{n,k} \in \R^n$ denotes the vector of size $n$ with all entries equal to zero, except for the $k$-th entry, which is equal to $1$, and 
\begin{equation}
    \cantor(u) := \sum_{i=0}^\infty  \frac{2 u_i +1}{4^{i}}, \quad \forall u \in \binsymb^\N,
\end{equation}
The choice of $\cantor$ as an encoding relies on the fact that we can extract $u_1$ from $\cantor(u)$ with operations that can be implemented with neurons, as follows. Define $\CReLU : \realx \mapsto \max(\min(\realx,1), 0) = \ReLU(\realx) - \ReLU(\realx-1)$. Then, for all $u \in \binsymb^\N$, we have
\begin{equation}\label{eq:extracting-symbol-from-encoding}
    u_1 = \CReLU(4 \cantor(\sequ) - 2),
\end{equation}
i.e., the operation of reading of the first bit can be implemented in a \NN. Following the previous discussion, the \NN $\nn$ must satisfy
\begin{equation}
    \rnnHidSeq[t] = \begin{pmatrix}
        1_{n_Q, \trajState{}{t}{}} \\
        \cantor(\trajTape{L}{t}{}) \\
        \cantor(\trajTape{R}{t}{})
    \end{pmatrix} = \nn(\rnnHidSeq[t-1]) = \nn\begin{pmatrix}
        1_{n_Q, \trajState{}{t-1}{}} \\
        \cantor(\trajTape{L}{{t-1}}{}) \\
        \cantor(\trajTape{R}{{t-1}}{})
    \end{pmatrix}, \quad \forall t \in \N_0.
\end{equation}
In order to understand better how such a \NN can be constructed, we need to understand how the Turing machine $\tm$ transforms $\trajState{}{t-1}{}$, $\trajTape{L}{{t-1}}{}$ and $\trajTape{R}{{t-1}}{}$ into $\trajState{}{t}{}$, $\trajTape{L}{t}{}$ and $\trajTape{R}{t}{}$. This transformation process can be summarized as follows:
\begin{enumerate}[label = (\alph*)]
    \item The Turing machine $\tm$ reads the first symbol $\symb \in \binsymb$ of the sequence $\trajTape{R}{{t-1}}{}$ (which is equivalent to read the symbol written in the cell of the tape that is located under the head of the Turing machine).
    \item The Turing machine $\tm$ applies its transition function $\transFunc$ to $(\trajState{}{t-1}{}, \symb)$. This delivers 3 outputs: a new state $\trajState{}{t}{} \in Q$, a new symbol $\symb \in \binsymb$ to be written in the cell under scan, and a head movement direction (left, right, or stay in place). 
    \item As a consequence of the previous step, the sequences $\trajTape{L}{{t-1}}{}$ and $\trajTape{R}{{t-1}}{}$ are modified as follows:
    \begin{enumerate}[label = (\roman*)]
        \item If the movement is $0$, then the Turing machine writes the symbol $\symb$ in the cell under scan, and does not move the head. In this case,
        \begin{equation}\label{eq:update of the left and right parts of the tape when movement is 0}
            \trajTape{L}{t}{} = \trajTape{L}{{t-1}}{}, \quad \trajCell{R}{t}{}{1} = \symb, \quad  \text{and} \ \trajCell{R}{t}{}{i} = \trajCell{R}{{t-1}}{}{i}, \quad \forall i \geq 2.
        \end{equation}
        \item If the movement is $-1$, then the Turing machine writes the symbol $\symb$ in the cell under scan, and moves the head one position to the left. In this case, we need to first modify the first symbol of the right part into $\symb$. We denote the consequently modified right part of the tape $\trajTapeTilde{R}{t}{}$, which hence satisfies 
        \begin{equation}\label{eq:intermediate update of the right part of the tape when movement is -1}
            \trajCellTilde{R}{t}{}{1} = \symb, \quad \trajCellTilde{R}{t}{}{i} = \trajCellTilde{R}{{t-1}}{}{i}, \quad \forall i \geq 2.
        \end{equation}
        Then, we need to remove the first symbol of the left part, and to add it to the right part. Hence, we have
        \begin{equation}\label{eq:update of the left part of the tape when movement is -1}
            \trajCell{L}{t}{}{i} = \trajCell{L}{{t-1}}{}{{i+1}}, \quad \forall i \geq 1,
        \end{equation}
        and 
        \begin{equation}\label{eq:update of the right part of the tape when movement is -1}
            \trajCell{R}{t}{}{1} = \trajCell{L}{{t-1}}{}{1}, \quad \trajCell{R}{t}{}{i} = \trajCellTilde{R}{t}{}{{i-1}}, \quad \forall i \geq 2.
        \end{equation}
        \item If the movement is $1$, then the Turing machine writes the symbol $\symb$ in the cell under scan, and moves the head one position to the right. In this case, we need to remove the first symbol of the right of the tape, and to add the symbol $\symb$ to the left part. Hence, we have
        \begin{equation}\label{eq:update of the right part of the tape when movement is 1}
            \trajCell{R}{t}{}{i} = \trajCell{R}{{t-1}}{}{{i+1}}, \quad \forall i \geq 1,
        \end{equation}
        and 
        \begin{equation}\label{eq:update of the left part of the tape when movement is 1}
            \trajCell{L}{t}{}{1} = \symb, \quad \trajCell{L}{t}{}{i} = \trajCell{L}{t}{}{{i-1}}, \quad \forall i \geq 2.
        \end{equation}
    \end{enumerate}
\end{enumerate}
Then, equivalently, the neural network $\nn$ needs to implement the following transformation to be applied to $\rnnHidSeq[t-1]$.
\begin{enumerate}[label = (\alph*)]
    \item The neural network $\nn$ extracts the symbol $\symb = \trajCell{R}{{t-1}}{}{1} \in \binsymb$ from $\cantor(\trajTape{R}{{t-1}}{})$ by the operation (\ref{eq:extracting-symbol-from-encoding}).  
    \item The neural network $\nn$ mimics the transition function $\transFunc$ to determine the new state $\state \in A$, the symbol $\symb \in \binsymb$ to be written and the move $m \in \Mc$ to be made. We divide $\transFunc$ into three subfunctions $\transFunc_1$, $\transFunc_2$, $\transFunc_3$, such that
    \begin{equation}
        \transFunc(\state,\symb) = (\transFunc_\state(\state,\symb), \transFunc_\symb(\state,\symb), \transFunc_\move(\state,\symb)).
    \end{equation}
    We show how $\transFunc_\state$ can be simulated with neurons, the proof for the other 2 functions being analogous. We first define a function $\tilde \transFunc_\state : \{0,1\}^{n_Q+1} \to \{0,1\}^{n_Q}$ that mimics $\transFunc_\state$. This function is defined by 
    \begin{equation}
        \tilde \transFunc_\state \begin{pmatrix}
            1_{n_Q, \state} \\
            \symb \\
        \end{pmatrix} = 1_{n_Q, \transFunc_\state(\state,\symb)}.
    \end{equation}
    We now proceed to show that $\tilde \transFunc_\state$ can be implemented with neurons. Note that the input $(1_{n_Q,\state}, \symb)$ of $\tilde \transFunc_\state$ can take $2n_Q$ different values, that can be indexed by the integer $2q + \symb - 1 \in \{1, \ldots, 2n_Q\}$. The first step is to transform $(1_{n_Q,\state}, \symb)$ into $1_{2n_Q, 2q + \symb - 1}$. This is effected through the simple following affine transformation
    %  satisfying
    % \begin{equation}
    %     k(\state',\symb') = \begin{cases}
    %         2q'-1, & \text{if } \symb' = 0,\\
    %         2q', & \text{if } \symb' = 1.
    %     \end{cases}
    % \end{equation}
    % The first We cast the vector The first step is then to cast the input $(1_{n_Q,\state'}, \symb')$ into the one-hot vector $1_{2n_Q,k(\state',\symb')}$. This can be effected by the affine transformation
    \begin{equation}
        1_{2n_Q,2q+\symb - 1} = A \times \begin{pmatrix}
            1_{n_Q,\state}\\
            \symb
        \end{pmatrix} + b,
    \end{equation}
    where $A \in \{-1,0,1\}^{2n_Q \times (n_Q+1)}$ is such that
    \begin{align}
        A_{2i-1,i} &= A_{2i,i} = 1,\\
        -A_{2i-1,n_Q+1} &= A_{2i,n_Q+1} = 1,\\
        b_{2i} &= 1,   
    \end{align}
    for all $i \in \{1, \ldots, n_Q\}$, and all the other entries of $A$ and $b$ are equal to $0$. Once the affine transformation applied, we make a matrix multiplication that reproduces the function $\tilde \transFunc_\state$. This matrix multiplication is given by
    \begin{equation}
        \tilde \transFunc_\state \begin{pmatrix}
            1_{n_Q, \state} \\
            \symb \\
        \end{pmatrix} = W \times 1_{2n_Q,2q+\symb-1},
    \end{equation}
    where $W \in \{0,1\}^{n_Q \times 2n_Q}$ satisfies
    \begin{equation}
        W_{i,j} = \begin{cases}
            1, & \text{if } j = 2q+\symb-1, \ and \ i = \transFunc_\state(\state,\symb) \ for \ some \ (\state,\symb) \in Q \times \{0,1\}\\
            0, & \text{otherwise.}
        \end{cases}
    \end{equation}
    We conclude that $\tilde \transFunc_\state$ can be implemented with neurons through
    \begin{equation}
        \tilde \transFunc_\state \begin{pmatrix}
            1_{n_Q, \state} \\
            \symb \\
        \end{pmatrix} = W \times A \times \begin{pmatrix}
            1_{n_Q,\state}\\
            \symb
        \end{pmatrix} + b.
    \end{equation}
    The same goes for $\transFunc_\symb$ and $\transFunc_\move$, and therefore for $\transFunc$, that we implement through a function $\tilde \transFunc$. The output of $\tilde \transFunc$ is a vector of size $n_Q + 2$, where the first $n_Q$ coordinates correspond to the new state $\state'$, the next coordinate corresponds to the new symbol $\symb$ to be written, and the last coordinate corresponds to the movement $m \in \Mc$ that has been chosen.
    \item The neural network uses the output of $\tilde \transFunc$ to compute $\rnnHidSeq[t]$ as follows. The first $n_Q$ coordinates of $\rnnHidSeq[t]$ are set to $1_{n_Q, \state'}$. Then, the last two coordinates are calculated as follows, depending on the movement $m \in \Mc$ that has been chosen.
    \begin{enumerate}[label = (\roman*)]
        \item If $ m = 0$, the left part of the tape remains unchanged, so
        \begin{equation}
            \cantor(\trajTape{L}{t}{}) = \cantor(\trajTape{L}{{t-1}}{}).
        \end{equation}
        The first symbol of the right part of the tape is set to $\symb$. Following (\ref{eq:update of the left and right parts of the tape when movement is 0}), we have
        \begin{equation}
            \cantor(\trajTape{R}{t}{}) = \cantor(\trajTape{R}{{t-1}}{}) + \frac{2 \symb+1}{4} - \frac{2 \trajCell{R}{{t-1}}{}{1} + 1}{4} \cdot
        \end{equation}
        \item If $m = -1$, we need to `write' the symbol $\symb$ to the tape, and move the head one position to the left. Following (\ref{eq:intermediate update of the right part of the tape when movement is -1}), we get 
        \begin{equation}
            \cantor(\trajTapeTilde{R}{t}{}) = \cantor(\trajTape{R}{{t-1}}{}) + \frac{2 \symb+1}{4} - \frac{2 \trajCell{R}{{t-1}}{}{1} + 1}{4} \cdot
        \end{equation}
        Moreover, following (\ref{eq:update of the left part of the tape when movement is -1}) and (\ref{eq:update of the right part of the tape when movement is -1}), we have
        \begin{equation}
            \cantor(\trajTape{L}{t}{}) = 4\cantor(\trajTape{L}{{t-1}}{}) - 2\trajCell{L}{{t-1}}{}{1} - 1,
            % \overset{(a)}{=} 4\cantor(\trajTape{L}{{t-1}}{}) - 2\CReLU(4\cantor(\trajTape{L}{{t-1}}{})-2) - 1,
        \end{equation}
        and
        \begin{align}
            \cantor(\trajTape{R}{t}{}) &= \frac{1}{4}\cantor(\trajTapeTilde{R}{t}{}) + 2\trajCell{L}{{t-1}}{}{1} + 1.
            % \overset{(b)}{=} \frac{1}{4}\cantor(\trajTapeTilde{R}{t}{})+ 2\CReLU(4\cantor(\trajTape{L}{{t-1}}{})-2) + 1\\
            % &= \frac{1}{4}\cantor(\trajTape{R}{{t-1}}{}) + \frac{2 \symb+1}{16} - \frac{2 \symb + 1}{16} + 2\CReLU(4\cantor(\trajTape{L}{{t-1}}{})-2) + 1,
        \end{align}
        \item If $m = 1$, we need to `write' the symbol $\symb$ to the tape, and move the head one position to the right. Following (\ref{eq:update of the right part of the tape when movement is 1}), we have
        \begin{equation}
            \cantor(\trajTape{R}{t}{}) = 4\cantor(\trajTape{R}{{t-1}}{}) - 2\trajCell{R}{{t-1}}{}{1} - 1,
        \end{equation}
        and
        \begin{align}
            \cantor(\trajTape{L}{t}{}) &= \frac{1}{4}\cantor(\trajTape{L}{{t-1}}{}) + \frac{2 \symb+1}{4}.
        \end{align} 
    \end{enumerate}
    Note that all the operations above can be implemented with neurons, since they only involve addition, multiplication by constants and (\ref{eq:extracting-symbol-from-encoding}).
\end{enumerate}

This concludes the description of the \NN $\nn$, and hence the proof that Turing machines can be simulated by iterations of a \NN. We next move to the proof that \RNNs can simulate Turing machines with neural units.

\subsection{Simulation of \TMNUs with \RNNs}

\label{sec:simulation-turing-machines-neural-units-with-rnns}

Let $\tmnu = (n_Q,W_i,W_o,\transFunc,\commFunc)$ be a \TMNU. For $M>0$, we say that $\tmnu$ is $M$-bounded at $(\tapeIn, \neurIn) \in \domOut \tmnu$ if $S_\tmnu(\tapeIn, \neurIn) \leq M$. We define the $M$-domain of $\tmnu$ as
\begin{equation}
    \domOut_M \tmnu = \left\{(\tapeIn, \neurIn) \in \domOut \tmnu : S_\tmnu(\tapeIn, \neurIn) \leq M\right\}.
\end{equation}
In the sequel, we will show that for every given $M>0$, a \TMNU can be simulated by an \RNN over its $M$-domain. Specifically, we push the intuitions delivered by the simulation of Turing machines with \RNNs further, and show that \RNNs can simulate bounded \TMNUs. The proof is extremely similar. Indeed, the Turing machine part of a \TMNU is completely independent of the neural units, and therefore the simulation of the Turing machine part is exactly the same as in Section \ref{sec:simulation-turing-machines-rnns}. The only difference is that we need to additionally simulate the function $\commFunc$ with neurons. 
% As we will see, we will need a little extra information to simulate a given I\TMNU with an \RNN: we will need to know an upper bound of $S_\Phi(\bfx_0,\neurState_0)$. 
% For pedagogical purposes, we will give the construction of an \RNN simulating a bounded I\TMNU, i.e. an I\TMNU for which there exists an $M > 0$ such that $S_\Phi(\bfx_0,\neurState_0) \leq M$ for all $(\bfx_0, \neurState_0) \in \domOut \Phi$, and then we will turn to the general case.

% \subsubsection{Bounded I\TMNUs}


We first show how to simulate a TMNU over its $M$-domain by iterations of a \NN. Specifically, we will show that starting from 
\begin{equation}
    \rnnHidSeq[0] = \begin{pmatrix}
        \trajNeur{}{0}{}{} \\
        1_{n_Q, \trajState{}{0}{}} \\
        \cantor(\trajTape{L}{0}{}) \\
        \cantor(\trajTape{R}{0}{})
    \end{pmatrix} \in \R^{\neurDim + n_Q + 2},
\end{equation}
we can construct a neural network $\Lambda_M : \R^{\neurDim + n_Q + 2} \to \R^{\neurDim + n_Q + 2}$ and define the sequence $\rnnHidSeq[\cdot]$ by $\rnnHidSeq[t] = \Lambda_M(\rnnHidSeq[t-1])$, $t \in \N$, such that
\begin{equation}
    \rnnHidSeq[t] = \begin{pmatrix}
        \trajNeur{}{t}{}{} \\
        1_{n_Q, \trajState{}{t}{}} \\
        \cantor(\trajTape{L}{t}{}) \\
        \cantor(\trajTape{R}{t}{})
    \end{pmatrix} \in \R^{\neurDim + n_Q + 2}, \quad \forall t \in \N_0,
\end{equation}
under the assumption that $\|\trajNeur{}{t}{}{}\|_\infty \leq M$ for all $t \in \No$. Consider the neural network $\nn : \R^{n_Q +2} \to \R^{n_Q+2}$ defined in Section \ref{sec:simulation-turing-machines-rnns} to simulate a step of computation of a Turing machine. Then, the \NN $\Lambda_M : \R^{\neurDim + n_Q + 2} \to \R^{\neurDim + n_Q + 2}$ that simulates a step of computation of a Turing machine with neural units satisfies
\begin{equation}
    \Lambda_M\begin{pmatrix}
        \trajNeur{}{t}{}{}\\
        1_{n_Q, \trajState{}{t}{}}\\
        \cantor(\trajTape{L}{t}{})\\
        \cantor(\trajTape{R}{t}{})
    \end{pmatrix} = \begin{pmatrix}
        \commFunc(\trajState{}{t}{},\trajCell{R}{{t-1}}{}{1})(\trajNeur{}{{t-1}}{}{})\\
        \nn\begin{pmatrix}
            1_{n_Q, \trajState{}{{t-1}}{}}\\
            \cantor(\trajTape{L}{{t-1}}{})\\
            \cantor(\trajTape{R}{{t-1}}{})
        \end{pmatrix}\\
    \end{pmatrix}.
\end{equation}
where $\nn$ is defined as in Section \ref{sec:simulation-turing-machines-rnns}, we only need to construct a neural network $\nn_{\commFunc,M} : \R^{\neurDim + n_Q + 2} \to \R^\neurDim$ that simulates the function $\commFunc$, i.e., that satisfies
\begin{equation}
    \nn_{\commFunc,M}\begin{pmatrix}
        \trajNeur{}{t}{}{}\\
        1_{n_Q, \trajState{}{t}{}}\\
        \cantor(\trajTape{L}{t}{})\\
        \cantor(\trajTape{R}{t}{})
    \end{pmatrix} = \commFunc(\trajState{}{{t-1}}{},\trajCell{R}{{t-1}}{}{1})(\trajNeur{}{{t-1}}{}{}),
\end{equation}
under the assumption that $\|\trajNeur{}{t}{}{}\|_\infty \leq M$. We proceed to explain the construction of $\nn_\commFunc$. First, note that $\commFunc : \states \times \binsymb \to \neurFuncs$, where $\neurFuncs$ is the set of neural functions. We denote by $N \in \N$ the number of neural functions in $\rg(\commFunc) \subseteq \neurFuncs$, and fix an enumeration $f_1, \ldots, f_N$ fo $\rg(\commFunc)$. Then, $\commFunc$ can be simulated exactly as we have simulated the function $\transFunc_\state$ in Section \ref{sec:simulation-turing-machines-rnns}. Namely, we consider the function $\tilde \commFunc : \{0,1\}^{\nStates +1} \to \{0,1\}^N$ that satisfies
\begin{equation}
    \tilde \commFunc\begin{pmatrix}
        1_{n_Q, \state}\\
        \symb
    \end{pmatrix} = 1_{N, i},
\end{equation}
where $i$ is the index of the function $f_i \in \rg(\commFunc)$ such that $f_i = \commFunc(\state,\symb)$. $\tilde \commFunc$ is implemented with neurons exactly as $\tilde \transFunc_\state$ in Section \ref{sec:simulation-turing-machines-rnns}. There remains to apply the neural function $\commFunc(\state,\symb)$ to the neural state $\neurState$. To do so, we actually compute simultaneously $f(\neurState)$ for every $f \in \rg(\commFunc) \subseteq \neurFuncs$. This can be done with neurons through the following function
\begin{equation}
    F(\neurState) = \begin{pmatrix}
        f_1(\neurState)\\
        \vdots\\
        f_N(\neurState)
    \end{pmatrix},
\end{equation}
where $f_i \in \neurFuncs$ is the $i$-th neural function in $\rg(\commFunc) \subseteq \neurFuncs$. Once we have computed $F(\neurState)$, we can compute the new neural state $\neurState'$ by setting to zero all the coordinates of $F(\neurState)$ except for the coordinates corresponding to $f_i$, and them summing the contribution of every function (which will be zero for every function, except for $f_i$). Under the assumption that $\|\neurState\|_\infty \leq M$, this is done by applying in parallel the functions $\realx \mapsto \ReLU(\realx - M)$ and $\realx \mapsto \ReLU(-\realx - M)$ to every coordinate of $F(\neurState)$, except the coordinates of $f_i$, and taking the difference between the contributions of both parallelized computations. This is summarized by the following equation
\begin{equation}
    \tilde F(\neurState) := \begin{pmatrix}
        0_{(i-1)\neurDim}\\
        f_i(\omega)\\
        0_{(N-i)\neurDim}
    \end{pmatrix} = (1 \ -1) \times \ReLU \left(
        \begin{pmatrix}
            F(\neurState)\\
            - F(\neurState)
        \end{pmatrix} + M\left(1 - \sum_{\ell = id+1}^{(i+1)d}\begin{pmatrix}
            1_{Nd, \ell}\\
            1_{Nd, \ell}
        \end{pmatrix}\right)\right)
\end{equation}
Finally, we get $f_i(\neurState)$ by summing the coordinates, which is expressed by
\begin{equation}
    f_i(\neurState) = \sum_{j = 0}^{N-1} \begin{pmatrix}
        \tilde F_{jd + 1}(\neurState)\\
        \vdots\\
        \tilde F_{(j+1)d}(\neurState)
    \end{pmatrix}.
\end{equation}
    %     \ReLU\left(  + (1- 1_{N, \lceil i/d \rceil})M\right)\\
    %     \ReLU\left(-F(\neurState)  + (1- 1_{N, \lceil i/d \rceil})M\right)
    % \end{pmatrix}
% \end{equation}
This concludes the construction of the \NN $\nn_{\commFunc,M}$, and therefore the construction of the \NN $\Lambda_M$. We now show how to construct an \RNN $\rnn_M$ that simulates the \TMNU $\tmnu$ on its $M$-domain, based on the \NN $\Lambda_M$. This \RNN satisfies $\rnnInDim = \inDim$, $\rnnHidDim = \neurDim + \nStates + 2$ and $\rnnOutDim = \outDim$, such that
\begin{equation}
    \nn_h\begin{pmatrix}
        \rnnHid\\
        \rnnIn
    \end{pmatrix} = \Lambda_M\left(\rnnHid + \proji {\rnnHidDim} {} (W_i \times \rnnIn)\right), \quad (\rnnHid, \rnnIn) \in \rnnHidOpInSpace,
\end{equation}
and
\begin{equation}
    \nn_o(\rnnHid) = \begin{pmatrix}
        \outMat & \zeroMat_{\outDim, n_Q + 2}
    \end{pmatrix} \times \rnnHid, \quad \rnnHid \in \rnnHidSpace.
\end{equation}
Then, let $(\tapeIn,\neurIn) \in \domOut_M(\tmnu)$, and define $(\rnnInSeq[t])_{t \in \No}$ by $\rnnInSeq[0] = \neurIn$ and $\rnnInSeq[t] = 0$ for all $t \in \N$, and
\begin{equation}
    \rnnHidSeq[-1] = \begin{pmatrix}
        0_{\neurDim}\\
        1_{n_Q, 1}\\
        \cantor(0^\N)\\
        \cantor(\tapeIn)
    \end{pmatrix} \in \R^{\neurDim + n_Q + 2},
\end{equation}
we get
\begin{equation}
    \rnn_M\rnnInSeq[t] = W_o \times \trajNeur{}{t}{}{}, \quad \forall t \in \N_0. 
\end{equation}
Then, $\rnn_M$ simulates $\tmnu$ over $\domOut_M(\tmnu)$. Notably,
\begin{equation}
    \limi t \rnn_M\rnnInSeq[t] = \limFunc{\tmnu}(\tapeIn, \neurIn).
\end{equation}
We cast the above discussion into a formal Theorem.
\begin{theorem}(RNNs can simulate \TMNUs on their $M$-domain)\label{thm:rnns-can-simulate-tmnus-on-their-m-domain}
    Let $\tmnu$ be a \TMNU, and let $M > 0$. Then, there exists an \RNN $\rnn_M$ such that $\rnn_M$ simulates $\tmnu$ on its $M$-domain, i.e. for every $(\tapeIn, \neurIn) \in \domOut_M(\tmnu)$, we have
        \begin{equation}
            \rnn_M\rnnInSeq[t] = \trajFunc{\tmnu}(\tapeIn, \neurIn)[t], \quad \forall t \in \N_0.
        \end{equation}
\end{theorem}
In the next final section, we explain how to use this result in combination with the results of Section \ref{sec:TMNU-approximation-of-continuous-functions} to get the final result, namely that \RNNs can approximate continuous functions over compact sets.

% \subsubsection{General I\TMNUs}

% We now turn to general I\TMNUs. Consider an I\TMNU $\Phi$, and note that by definition, every $(\bfx_0, \neurState_0) \in \domOut \Phi$ satisfies
% \begin{equation}
%     S_\Phi(\bfx_0, \neurState_0) < \infty.
% \end{equation}
% Hence, every trajectory of the neural state of $\Phi$ is bounded, but, this bound may be nonuniform, i.e. it may depend on the initial state $(\bfx_0, \neurState_0)$.

% We now show how to simulate an arbitrary I\TMNU $\Phi$ on its domain $\domOut \Phi$ with an \RNN. For $(\bfx_0, \neurState_0) \in \domOut \Phi$, this simulation requires the \RNN to receive as input $2^{-M}$, where $M \in \N$ is an upper bound of $S_\Phi(\bfx_0, \neurState_0)$. Concretely, we construct a neural network $\tilde \Lambda_h : \R^{d + n_Q + 4} \to \R^{d + n_Q + 4}$ that incorporates a slight modification of the neural network $\Lambda_h$ defined in the previous section. Namely, we define $\tilde \Lambda$ so that the $d$ first coordinates of the hidden state $h[t] \in \R^{d + n_Q + 4}$ contain the neural state $\neurState \in \R^d$, the $n_Q + 2$ following coordinates are used to simulate the Turing machine part, and the last two coordinates store $2^{-M}$ and a variable that will be used to help the simulation of the function $\commFunc$. Concretely, we will design $\tilde \Lambda_h$ so that
% \begin{equation}
%     \tilde \Lambda_h\begin{pmatrix}
%         \neurState\\
%         1_{n_Q, \state}\\
%         \delta(\trajTape{L}{t}{})\\
%         \delta(\trajTape{R}{t}{})\\
%         2^{-M}\\
%         0
%     \end{pmatrix} = \begin{pmatrix}
%         \commFunc(\state,\trajCellTilde{R}{t}{}{1})(\neurState)\\
%         \nn_h\begin{pmatrix}
%             1_{n_Q, \state}\\
%             \delta(\trajTape{L}{t}{})\\
%             \delta(\trajTape{R}{t}{})
%         \end{pmatrix}\\
%             2^{-M}\\
%             0
%     \end{pmatrix}.
% \end{equation}


% that simulates a step of computation of a Turing machine with neural units, where the $d$ first coordinates store the neural state, the $n_Q + 2$ following coordinates simulate the Turing machine part exactly as in the last paragraph, and the last two coordinates are used to encode $M$. Concretely, we split $\Lambda_h$ into two parallel neural networks such that

\subsection{Approximation of continuous functions with \RNNs}

\label{sec:approximation-continuous-functions-rnns}
 
In this section, we show that \RNNs can approximate continuous functions over any compact set $\Omega \subseteq \R$. Let $f : \Omega \to \R$ be a continuous function, and let $\bfR \in \reprCun(f)$. By Theorem \ref{thm:continuous compact support is computably approx with neurons}, the set of continuous functions $\Cc(\Omega)$ is \ulcwn through the \TMNU $\limTMNU{\Continuous}$. This means that
\begin{equation}
    \limFunc{\limTMNU{\Continuous}}(\bfR, \neurIn) = \limi t \trajFunc{\limTMNU{\Continuous}}(\bfR, \neurIn)[t]  = f(\neurIn), \quad \forall \neurIn \in \Omega.
\end{equation}
Moreover, as $f$ is continuous and $\Omega$ is compact, there exists a constant $M \geq 1$ such that $|\neurIn|, \|f(\neurIn)\|_\infty + 1 \leq M$ for all $\neurIn \in \Omega$.  Hence, combining (\ref{eq:satcomp:thm:continuousL is computably approximability with neurons}) and Theorem \ref{thm:turing-machine-neural-units-infinite-approximation}, we have $\satComp{\limTMNU{\Continuous}}(\bfR, \neurIn) \leq \max\{1, |\neurIn| |f(\neurIn)| + 1\} \leq M$, i.e., $(\bfR,\neurIn) \in \domOut_M(\limTMNU{\Continuous})$, for all $\neurIn \in \Omega$. Therefore, we can apply Theorem \ref{thm:rnns-can-simulate-tmnus-on-their-m-domain} to the \TMNU $\limTMNU{\Continuous}$ over its $M$-domain. This means that there exists an \RNN $\rnn_M$ such that
\begin{equation}\label{eq:rnns can simulate tmnu on its m domain}
    \rnn_M\neurIn[t] = \trajFunc{\limTMNU{\Continuous}}(\bfR, \neurIn)[t], \quad \forall t \in \N_0, \quad \forall \neurIn \in \Omega.
\end{equation}
This observation leads to our main theorem.
\begin{theorem}(Main theorem: \RNNs can approximate continuous functions)\label{thm:rnns-can-approximate-continuous-functions}
    Let $f : \Omega \to \R$ be a continuous function. Then, there exists an \RNN $\rnn$ such that
    \begin{equation}
        \limi t \rnn\neurIn[t] = f(\neurIn), \quad \forall \neurIn \in \Omega.
    \end{equation}
\end{theorem}

The speed of convergence towards $f(\realx)$ allows characterizing complexity classes for continuous functions. Namely, given a function $\varphi : \N \to \N$, we say that a continuous function $f : \Omega \subseteq \R \to \R$ has time complexity $\varphi(n)$ if there exists a \RNN $\rnn$ such that
\[
    |\rnn \realx[\varphi(n)] - f(\realx)| \leq 2^{-n}, \ \ \forall n \in \N, \ \forall \realx \in \Omega.
\]
For $\varphi : \N \to \N$, we define $\Cc_{\RNN}[\varphi(n)]$ to be the set of continuous functions with time complexity $O(\varphi(n))$. Note that thanks to (\ref{eq:rnns can simulate tmnu on its m domain}) we get that 
\begin{equation}
     f \in \Cc_{\RNN}[\infTimeComp{\limTMNU{\Continuous}}(\bfR, \neurIn)[n]]
\end{equation}
 Then, from the bounds on the time complexity given at the end of Section \ref{sec:TMNU-approximation-of-continuous-functions}, we get that $f_P \in \Cc_{\RNN}[n]$, for all $P \in \R[X]$. Moreover, for $C^\infty$ functions over $[-1,1]$ satisfying $\|f^{(n)}\|_\infty \leq C n!$ for all $n \in \N$, we have
\begin{equation}
    f \in \Cc_{\RNN}\left[n^4 \log^2(n) \right].
\end{equation}
We leave open the question of the optimality of the rate $n^4 \log^2(n)$, and of the complexity classes associated with other classes of continuous functions.
% Namely, every polynomial is in the complexity class $O(t^2)$.
% For continuous functions, the complexity class heavily depends on its regularity properties. For example, if $f \in C^\infty([-1,1])$, we get by Chebychev-Lagrange interpolation that
% \[
%     f \in \Cc_{\RNN}\left[ n^{8} \log^8(n)  \left(n + \log\left(\frac{\|f^{(n)}\|_\infty}{n!}\right)\right)^4\right].
% \]
% For instance, if $\|f^{(n)}\|_\infty \leq n!$ for all $n \in \N$, we get 
% \[
%     f \in \Cc_{\RNN}\left[ n^{12} \log^8(n) \right].
% \]
% We leave open the question of the optimality of the rate $n^{12}\log^8(n)$.

==> tikzlibraryipe.code.tex <==

% Copyright (C) 2016  Joseph Rabinoff

% ipe2tikz is free software; you can redistribute it and/or modify it under
% the terms of the GNU General Public License as published by the Free
% Software Foundation; either version 3 of the License, or (at your option)
% any later version.

% ipe2tikz is distributed in the hope that it will be useful, but WITHOUT ANY
% WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the GNU General Public License for more
% details.

% You should have received a copy of the GNU General Public License along with
% ipe2tikz; if not, you can find it at "http://www.gnu.org/copyleft/gpl.html",
% or write to the Free Software Foundation, Inc., 675 Mass Ave, Cambridge, MA
% 02139, USA.


% ipe compatibility TikZ styles

\usetikzlibrary{arrows.meta}

\makeatletter

% These should behave almost exactly like ipe arrows.  They disable correcting
% for the miter length and line width.  This is important for visual consistency
% with ipe, since ipe arrows get much larger when the line width is increased.
% They also use the line join and cap styles from the main path.  These are very
% simple arrows: there is no harpoon version, and the convex hull computation is
% sloppy.

\pgfdeclarearrow{
  name = ipe _linear,
  defaults = {
    length = +1bp,
    width  = +.666bp,
    line width = +0pt 1,
  },
  setup code = {
    % Control points
    \pgfarrowssetbackend{0pt}
    \pgfarrowssetvisualbackend{
      \pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \pgfarrowssetlineend{\pgfarrowlength}
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \fi
    \pgfarrowssettipend{\pgfarrowlength}
    % Convex hull
    \pgfarrowshullpoint{\pgfarrowlength}{0pt}
    \pgfarrowsupperhullpoint{0pt}{.5\pgfarrowwidth}
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{0pt}{.5\pgfarrowwidth}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth}}
    \pgfusepathqstroke
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
  },
}


\pgfdeclarearrow{
  name = ipe _pointed,
  defaults = {
    length = +1bp,
    width  = +.666bp,
    inset  = +.2bp,
    line width = +0pt 1,
  },
  setup code = {
    % Control points
    \pgfarrowssetbackend{0pt}
    \pgfarrowssetvisualbackend{\pgfarrowinset}
    \pgfarrowssetlineend{\pgfarrowinset}
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength}
    \fi
    \pgfarrowssettipend{\pgfarrowlength}
    % Convex hull
    \pgfarrowshullpoint{\pgfarrowlength}{0pt}
    \pgfarrowsupperhullpoint{0pt}{.5\pgfarrowwidth}
    \pgfarrowshullpoint{\pgfarrowinset}{0pt}
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowinset
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{.5\pgfarrowwidth}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowinset}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth}}
    \pgfpathclose
    \ifpgfarrowopen
      \pgfusepathqstroke
    \else
      \ifdim\pgfarrowlinewidth>0pt\pgfusepathqfillstroke\else\pgfusepathqfill\fi
    \fi
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \the\pgfarrowinset,%
    \ifpgfarrowopen o\fi%
  },
}


% For correcting minipage width in stretched nodes
\newdimen\ipeminipagewidth
\def\ipestretchwidth#1{%
  \pgfmathsetlength{\ipeminipagewidth}{#1/\ipenodestretch}}

\tikzstyle{ipe import} = [
  % General ipe defaults
  x=1bp, y=1bp,
%
  % Nodes
  ipe node stretch/.store in=\ipenodestretch,
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe node/.style={
    anchor=base west, inner sep=0, outer sep=0, scale=\ipenodestretch
  },
%
  % Use a special key for the mark scale, so that the default can be overriden.
  % (This doesn't happen with the scale= key; those accumulate.)
  ipe mark scale/.store in=\ipemarkscale,
%
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
%
  ipe mark normal, % Set default
%
  ipe circle/.pic={
    \draw[line width=0.2*\ipemarkscale]
      (0,0) circle[radius=0.5*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe disk/.pic={
    \fill (0,0) circle[radius=0.6*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe fdisk/.pic={
    \filldraw[line width=0.2*\ipemarkscale]
      (0,0) circle[radius=0.5*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe box/.pic={
    \draw[line width=0.2*\ipemarkscale, line join=miter]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) rectangle
      ( .5*\ipemarkscale, .5*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe square/.pic={
    \fill
      (-.6*\ipemarkscale,-.6*\ipemarkscale) rectangle
      ( .6*\ipemarkscale, .6*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe fsquare/.pic={
    \filldraw[line width=0.2*\ipemarkscale, line join=miter]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) rectangle
      ( .5*\ipemarkscale, .5*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe cross/.pic={
    \draw[line width=0.2*\ipemarkscale, line cap=butt]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) --
      ( .5*\ipemarkscale, .5*\ipemarkscale)
      (-.5*\ipemarkscale, .5*\ipemarkscale) --
      ( .5*\ipemarkscale,-.5*\ipemarkscale);
    \coordinate () at (0,0);
  },
%
  % Arrow sizes (for TikZ arrows)
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=1},
  ipe arrow tiny/.style={scale=.4},
  ipe arrow small/.style={scale=.7},
  ipe arrow large/.style={scale=1.4},
  ipe arrow normal,
  /tikz/.cd,
%
  % Approximations to ipe arrows
  % Put in a style to allow to reset default scale when "ipe arrow normal" is
  % changed.  I think this is the only way, since all the parameters to arrows
  % are expanded when the tip is declared.
  ipe arrows/.style={
    ipe normal/.tip={
      ipe _pointed[length=1bp, width=.666bp, inset=0bp,
                   quick, ipe arrow normal]},
    ipe pointed/.tip={
      ipe _pointed[length=1bp, width=.666bp, inset=0.2bp,
                   quick, ipe arrow normal]},
    ipe linear/.tip={
      ipe _linear[length = 1bp, width=.666bp,
                  ipe arrow normal, quick]},
    ipe fnormal/.tip={ipe normal[fill=white]},
    ipe fpointed/.tip={ipe pointed[fill=white]},
    ipe double/.tip={ipe normal[] ipe normal},
    ipe fdouble/.tip={ipe fnormal[] ipe fnormal},
    % These should maybe use [bend], but that often looks bad unless it's on an
    % actual arc.
    ipe arc/.tip={ipe normal},
    ipe farc/.tip={ipe fnormal},
    ipe ptarc/.tip={ipe pointed},
    ipe fptarc/.tip={ipe fpointed},
  },
  ipe arrows, % Set default sizes
]

% I'm not sure how to do this in a .style, since the #args get confused.
\tikzset{
  rgb color/.code args={#1=#2}{%
    \definecolor{tempcolor-#1}{rgb}{#2}%
    \tikzset{#1=tempcolor-#1}%
  },
}

\makeatother

\endinput

